Uniting Nesterov and Heavy Ball Methods for Uniform Global Asymptotic Stability of the Set of Minimizers

We propose a hybrid control algorithm that guarantees fast convergence and uniform global asymptotic stability of the unique minimizer of a continuously differentiable, convex objective function. The algorithm, developed using hybrid system tools, employs a uniting control strategy, in which Nesterov's accelerated gradient descent is used "globally" and the heavy ball method is used "locally," relative to the minimizer. Without knowledge of its location, the proposed hybrid control strategy switches between these accelerated methods to ensure convergence to the minimizer without oscillations, with a (hybrid) convergence rate that preserves the convergence rates of the individual optimization algorithms. We analyze key properties of the resulting closed-loop system including existence of solutions, uniform global asymptotic stability, and convergence rate. Additionally, stability properties of Nesterov's method are analyzed, and extensions on convergence rate results in the existing literature are presented. Numerical results validate the findings and demonstrate the robustness of the uniting algorithm.

==> Sections/Abstract.tex <==
\begin{abstract}
	We propose hybrid control algorithms that guarantee fast convergence and uniform global asymptotic stability of the set of minimizers of a convex objective function. The algorithms, developed using hybrid system tools, employ a uniting control strategy to ensure convergence to the set of minimizers without oscillations, with (hybrid) convergence rates that preserve the convergence rates of the individual optimization algorithms.
	The first such hybrid control algorithm unites two standard heavy ball algorithms, one used globally and another used locally, with properly designed gravity and friction parameters. The subsequent two hybrid control algorithms, for strongly and nonstrongly convex objective functions, respectively, unite Nesterov's accelerated gradient descent globally and the heavy ball method locally. We analyze key properties of the resulting closed-loop systems including existence of solutions, uniform global asymptotic stability, and convergence rate. Additionally, attractivity properties of Nesterov's accelerated gradient descent are analyzed, and extensions on convergence rate results in the existing literature are presented. Numerical results validate the findings. 
\end{abstract}

==> Sections/DerivationsOfSets.tex <==
\section{Derivation of Sets $\U_0$, $\T_{1,0}$, and $\T_{0,1}$ from \Cref{sec:NonstronglyConvexNest}}
\label{sec:DerivOfSets}


%The set $\U_0$ is contained in the basin of attraction induced by $\hczero$, due to the global attractivity property guaranteed by \cref{thm:GAS-HBF}.



==> Sections/DynamicalHBF.tex <==
\section{{\color{red}Proofs of Heavy Ball Results}}
\label{sec:DynamicalHBF}
%Since this paper proposes uniting algorithms which utilize the heavy ball method as the local optimization algorithm, this section presents results on nominal properties for this algorithm. As mentioned in \Cref{sec:Intro}, the dynamical system for the heavy ball method is defined via \cref{eqn:HBF}. Let $\xi := \xp_1$ and $\dot{\xi} = \xp_2$. Then, \cref{eqn:HBF} can be reinterpreted as a plant, in \cref{eqn:HBFplant-dynamicsTR}, and a control algorithm in \cref{eqn:StaticStateFeedbackLawLocal}.
%In \cite{8815316}, it was proved that uniting individual heavy ball algorithms -- one with small $\lambda$ globally and one with large $\lambda$ locally, yields fast convergence and global asymptotic stability of the set of minimizers. 
	

%The following lemma, from \cite{polyak2017lyapunov}, summarizes some of the results of Lyapunov theory from an optimization perspective, for both strongly convex and nonstrongly convex functions $L$.
%
%\begin{lemma}
%	\label{lemma:LyapunovOptimization}
%	Let $F_P$ be defined via \cref{eqn:HBFplant-dynamicsTR}. Furthermore, let $L$ satisfy \cref{ass:Lipschitz}. Let $\dot{V}(\xp) = \langle \nabla V(\xp),F_P(\xp,u) \rangle$, and assume there exists a function $\mathcal{W}$ such that $-\dot{V}(\xp) \geq \mathcal{W}(\xp) \geq 0$ for all $\xp \in C$. Then the following statement holds true:
%	\begin{enumerate}[label={(L\arabic*)},leftmargin=*]
%%		\item \label{item:LyapunovOptimizationOne} Assume $\mathcal{W}$ is convex. Let $\xp : \dom \xp \in \reals^{2n}$ be locally absolutely continuous and such that $\rge \xp \subset C$. For each $T \in \dom \xp$
%%		\begin{equation*}
%%		\mathcal{W}(\overline{\xp}(T)) \leq \frac{V(\xp(0)) - V(\xp(T))}{T}
%%		\end{equation*}
%%		where $\overline{\xp}(T) = \frac{1}{T}\int_{0}^{T}\xp(t)dt$.
%		\item \label{item:LyapunovOptimizationTwo} If $\mathcal{W}(\xp(t)) \geq \varphi V(\xp(t))$, $\varphi > 0$, holds for all $\xp \in \reals^{2n}$ and $t \geq 0$, then
%		\begin{equation} \label{eqn:ExpConvergenceProperty}
%			V(\xp(t)) \leq V(\xp(0)) \exp(-\varphi t)
%		\end{equation}
%		 holds for all $t \geq 0$.
%	\end{enumerate}
%\end{lemma}
%
%\begin{proof}
%	Since $L$ is Lipschitz continuous, by \cref{ass:Lipschitz}, and since $L$ is bounded below, since $L$ is (nonstrongly) convex by \cref{ass:LisNSCVX}, then $V$, defined via \cref{eqn:LyapunovHBF} is Lipschitz continuous and bounded below.
%	
%%	To prove item \ref{item:LyapunovOptimizationOne}: Integrating the inequality $-\dot{V}(\xp) \geq \mathcal{W}(\xp)$  from $0$ to $T$ for the given locally absolutely continuous $\xp$ and $T \in \dom \xp$, we obtain
%%	\begin{equation}
%%	\int_{0}^{T}\mathcal{W}(\xp(t))dt \leq V(\xp(0)) - V(\xp(T)).
%%	\end{equation}
%%	Since $\mathcal{W}$ is convex, then due to Jensen's inequality \footnote{Jensen's inequality is $\varphi \left(\frac{1}{b-a} \int_{a}^{b} f(x)dx\right) \leq \frac{1}{b-a} \int_{a}^{b} \varphi\left(f(x)\right)dx$, where $a,b \in \reals$, $f : [a,b] \rightarrow \reals$ is a nonnegative, Lebesgue-integrable function, and $\varphi$ is a convex function on the real line.},
%%	\begin{align*}
%%	\mathcal{W}(\overline{\xp}(T)) & = \mathcal{W} \left(\frac{1}{T} \int_{0}^{T}\xp(t)dt\right) \leq  \frac{1}{T} \int_{0}^{T}\mathcal{W} \left(\xp(t)\right)dt\\
%%	& \leq \frac{1}{T}V(\xp(0)) - V(\xp(T)).
%%	\end{align*}	
%	To prove item \cref{item:LyapunovOptimizationTwo}: Multiplying $-\dot{V}(\xp) \geq \varphi V(\xp)$ by $-1$ and applying Gr\"{o}nwall's inequality yields \cref{eqn:ExpConvergenceProperty}.
%\end{proof}
%
%%We impose the following assumption on $L$ for some of the results below.
%
%% Put the last part of Theorem 3 from Polyak here!
%The following theorem, based on \cite{polyak2017lyapunov}, gives an exponential convergence rate for functions $L$ which satisfy \cref{ass:LisCVX}, and is derived from \cref{lemma:LyapunovOptimization}.
%
%\begin{theorem}[Convergence rate of the heavy ball method, for strongly convex $L$] \label{thm:HBFConvergenceRateSC}
%	Let $L$ satisfy \cref{ass:LisCVX}. Then, each maximal solution $t \mapsto (\xp_1(t),\xp_2(t))$ of \cref{eqn:HBFplant-dynamicsTR}-\cref{eqn:StaticStateFeedbackLawLocal} satisfies
%	\begin{equation} \label{eqn:ExpDistToMin}
%		L(\xp_1(t)) - L^* \leq (L(\xp_1(0)) - L^*) \exp \left(-2 \mu t \right)
%	\end{equation}
%	for all $t \geq 0$, where $\mu > 0$.
%\end{theorem}
%
%\begin{proof}
%	Since, by assumption \cref{ass:LisCVX}, $L$ is strongly convex, then this implies that $L$ also satisfies the Polyak-{\L}ojasiewicz inequality, which is a weaker condition than strong convexity \cite{8854991} \cite{karimi2016linear}. The Polyak-{\L}ojasiewicz inequality is defined as
%	\begin{equation} \label{eqn:Polyak-Lojasiewicz}
%		\left|\nabla L(\xp_1(t))\right|^2 \geq 2 \mu (L(\xp_1(t)) - L^*), \quad \mu > 0.
%	\end{equation}
%	Taking $\mathcal{W}(\xp) := \left|\nabla L(\xp_1)\right|^2$, $V(\xp) := (L(\xp_1) - L^*)$, and $\varphi := 2 \mu$, then by \cref{lemma:LyapunovOptimization}, each maximal solution $t \mapsto (\xp_1(t),\xp_2(t))$ of \cref{eqn:HBF} satisfies \cref{eqn:ExpConvergenceProperty} for all $t \geq 0$. This implies that each solution $t \mapsto (\xp_1(t),\xp_2(t))$ of \cref{eqn:HBF} also satisfies \cref{eqn:ExpDistToMin} for all $t \geq 0$. 
%\end{proof}




%The following theorem, from \cite{polyak2017lyapunov}, gives the convergence rate of $\frac{1}{t}$ for the heavy ball method, when $L$ is nonstrongly convex. To prove it, we will use Lemma \ref{lemma:LyapunovOptimization} and employ the following Lyapunov function, which was also proposed in \cite{polyak2017lyapunov}. 
%
%\begin{equation}\label{eqn:LyapunovPolyak}
%V(\xp) := \left(L(\xp_1) - L(\A_1) \right) + \frac{\lambda^2}{2\gamma} \left|\left|\xp_1 \right|_{\A_1} + \frac{1}{\lambda}\xp_2 \right|^2
%\end{equation}
%%Since by item \ref{item:minimizer} of Assumption \ref{ass:MJAssumptions}, $\xp_1^* = 0$ and $L^* = 0$, this yields
%%\begin{equation}\label{eqn:LyapunovPolyakMinZero}
%%V(\xp) := L(\xp_1) + \frac{\lambda^2}{2\gamma} \left|\xp_1 + \frac{1}{\lambda}\xp_2 \right|^2
%%\end{equation}
%
%\begin{theorem} (Convergence rate of the heavy ball method, when $L$ is nonstrongly convex)
%	\label{thm:ConvergenceRateHBFNSC}
%	Let $L$ satisfy Assumptions \ref{ass:MJAssumptions}, \ref{ass:LisNCVX}, and \ref{ass:CompactAndConnected}, and let $\lambda > 0$. Then, each maximal solution $t \mapsto (\xp_1(t),\xp_2(t))$ of the heavy ball algorithm, defined via \eqref{eqn:HBF_CTDynamics}, satisfies
%	\begin{equation} \label{eqn:Estimate}
%		L(\overline{\xp}_1(T)) - L(\A_1) \leq \frac{V(\xp(0)) - V(\xp(T))}{\lambda T}
%	\end{equation}
%	for all $\xp \in \reals^{2n}$, where the bound in \eqref{eqn:Estimate} is satisfied for each $T \in \dom \xp$.
%\end{theorem}
%
%\begin{proofnew}
%	$V$, defined via \eqref{eqn:LyapunovPolyak}, is bounded below as follows:
%	\begin{equation} \label{eqn:LowerBoundVPolyak}
%		\frac{\lambda^2}{2\gamma} \left| \left|\xp_1 \right|_{\A_1} + \frac{1}{\lambda} \xp_2\right|^2 \leq V(\xp)
%	\end{equation}
%	Since $V$ satisfies \eqref{eqn:LowerBoundVPolyak}, and since $V$ is convex, due to $L$ being convex by Assumption \ref{ass:LisNCVX}, then for each $\xp \in \reals^{2n}$, $\dot{V}$ satisfies
%	\begin{align} \label{eqn:dotVPolyak}
%	\dot{V}(\xp) = & \langle \nabla V(\xp),f(\xp,u) \rangle \nonumber\\
%%	& = \matt{\nabla L(\xp) + \frac{\lambda^2}{\gamma}\left(\left|\xp_1 \right|_{\A_1} + \frac{1}{\lambda}\xp_2 \right) \ \frac{\lambda}{\gamma}\left(\left|\xp_1 \right|_{\A_1} + \frac{1}{\lambda}\xp_2 \right)} 
%%	\matt{\xp_2 \\ -\lambda \xp_2 - \gamma \nabla L(\xp_1)} \nonumber \\
%	= & \xp_2 \nabla L(\xp_1) + \frac{\lambda^2 \xp_2}{\gamma}\left(\left|\xp_1 \right|_{\A_1}  + \frac{1}{\lambda}\xp_2 \right) \nonumber\\
%	& - \frac{\lambda^2 \xp_2}{\gamma}\left(\left|\xp_1 \right|_{\A_1}  + \frac{1}{\lambda}\xp_2 \right)\nonumber\\
%	\quad & - \lambda \nabla L(\xp_1)\left(\left|\xp_1 \right|_{\A_1} + \frac{1}{\lambda}\xp_2 \right) \nonumber \\
%	= & \nabla L(\xp_1) \left[\xp_2 - \lambda \left(\left|\xp_1 \right|_{\A_1} + \frac{1}{\lambda}\xp_2 \right)\right] \nonumber \\
%	= & -\lambda \langle \nabla L(\xp_1),\left|\xp_1 \right|_{\A_1} \rangle \leq 0.
%	\end{align}
%	since $\lambda > 0$. Due to the convexity of $L$, then $\mathcal{W}$ can be chosen as $\mathcal{W}(\xp) := \lambda (L(\xp_1) - L(\A_1))$, for each $\xp \in \reals^{2n}$.  Consequently, item \ref{item:LyapunovOptimizationOne} of Lemma \ref{lemma:LyapunovOptimization} yields 
%	\begin{equation}
%		L(\overline{\xp}_1(T)) - L(\A_1) \leq \frac{V(\xp(0)) - V(\xp(T))}{\lambda T}
%	\end{equation}
%	for the heavy ball algorithm defined via \eqref{eqn:HBF_CTDynamics}.
%\end{proofnew}

==> Sections/DynamicalNesterov.tex <==
\section{{\color{red}Proofs of Results on Nesterov's Accelerated Gradient Descent}}
\label{sec:DynamicalNesterov}

%As was mentioned in \Cref{sec:Intro}, a second-order ODE for Nesterov's accelerated gradient descent, defined via \cref{eqn:MJODENCVX}, is presented in \cite{muehlebach2019dynamical}. The constant $M_{\zeta} := M\zeta^2$ consists of $\zeta > 0$, which determines the scaling of solutions to \cref{eqn:MJODENCVX} in time, and $M > 0$, which is the Lipschitz constant for $\nabla L$. For simplicity of analysis in \cite{muehlebach2019dynamical}, the authors set $\zeta = 1$. We, however, present results in this paper using the more general $\zeta > 0$. The ODE in \cref{eqn:MJODENCVX} is time-varying, where {\color{red}properly chosen $\bar{d}$ and $\bar{\beta}$ depend on $t$}. Namely, we use \cref{ass:LisNSCVX} in the results to follow. Although the authors in \cite{muehlebach2019dynamical} also assume that $\xp_1^* = 0$ and $L^* = 0$, we relax this assumption in the following analysis.  
%
%The corresponding continuous-time dynamics for $\xp := (\xp_1, \xp_2) \in \reals^{2n}$ are
%\begin{subequations}
%	\begin{align}
%		\dot{\xp}_1 & = \nabla T(\xp_2)\\
%		\dot{\xp}_2 & = - \frac{1}{M_{\zeta}} \nabla L(\xp_1) + L_{NP}(\xp,t)
%	\end{align}
%\end{subequations}
%where $\xi := \xp_1$ and $\dot{\xi} = \xp_2$. The real-valued, continuously differentiable function $T(\xp_2)$ represents the kinetic energy, and the continuous, real-valued function $L_{NP}(\xp,t)$ represents the non-potential forces. These functions are defined as
%\begin{subequations}
%	\begin{align}
%		T(\xp_2) & := \frac{1}{2} \left|\xp_2\right|^2\\
%		L_{NP}(\xp,t) & := -2\bar{d}(t)\xp_2 - \frac{1}{M_{\zeta}}\left( \nabla L(\xp_1 + \bar{\beta}(t) \xp_2)  - \nabla L(\xp_1)\right)
%	\end{align}
%\end{subequations}
%which
%%, when employing the state $\tau$ to capture ordinary time as a state variable, 
%leads to 
%\begin{equation}\label{eqn:MJ_CTDynamicsNCVX}
%\matt{\dot{\xp_1} \\ \dot{\xp_2}} = \matt{\xp_2 \\ -2\bar{d}(t)\xp_2 - \frac{1}{M_{\zeta}} \nabla L(\xp_1 + \bar{\beta}(t) \xp_2) \\ 1} =: f(\xp,t)
%\end{equation}
%for all $(\xp_1, \xp_2) \in \reals^{2n}$ and for all $t \in \reals_{\geq 0}$. 


==> Sections/HBF-HBF.tex <==
\section{Uniting Specific Accelerated Gradient Methods}
\label{sec:SpecificCases}
In this section, we present specific cases of uniting algorithms, which fit into the framework described in \Cref{sec:ModelingUF} and which use combinations of the heavy ball algorithm and Nesterov's algorithm. For each case, we present the data of the hybrid closed-loop system $\HS$ resulting from the specific combination of optimization algorithms, and then we present the main result for such a combination. We start first with the simplest case, which unites local and global heavy ball algorithms. 

\subsection{Uniting Heavy Ball Algorithms}
\label{sec:HBF-HBF}
In this section, we present a specific case of the framework in \Cref{sec:ModelingUF} which unites two standard heavy ball algorithms, namely, one heavy ball algorithm with small $\lambda$ used far from the minimizer and the other with large $\lambda$ used near the minimizer. For this specific case, \cref{ass:LisNSCVX} holds. 

The static state-feedback laws used for $\HS_{\xlogic}$ are
\begin{equation} \label{eqn:HBF_HCQ}
	u = \hcq(\hp_{\xlogic}(\xp)) = -\lambda_{\xlogic} \xp_2 - \gamma_{\xlogic} \nabla L(\xp_1)
\end{equation}
For each $\xlogic \in \xlogicSpace := \{0,1\}$. {\color{red}The state $\tau$ is not needed because the heavy ball algorithm is time-invariant, as shown in \cref{eqn:HBF}.} The parameters $\lambda_{\xlogic} > 0$ and $\gamma_{\xlogic} > 0$ should be designed for each $\xlogic \in \xlogicSpace$, to achieve fast convergence without oscillations nearby the minimizer. 
%The algorithm defined by $\hcone$ plays the role of the global algorithm in uniting control (see, e.g., \cite{220}), while the algorithm defined by $\hczero$ plays the role of the local algorithm. 
For the individual heavy ball algorithms, $\hp_{\xlogic}$ is defined as
\begin{equation} \label{eqn:HBF-HBFFunctionH}
	\hp_0(\xp) = \hp_1(\xp) := \matt{\xp_2\\ \nabla L(\xp_1)}
\end{equation}
where $\hp_0$ corresponds to the output for the local heavy ball algorithm and $\hp_1$ corresponds to the output for the global heavy ball algorithm. 
%The algorithm for $q = 1$ will be designed to achieve fast convergence and is referred to as global. The algorithm for $q = 0$ will be designed to achieve stable convergence near the minimizer and is referred to as local. 
%Due to $\xlogic$ jumping between 0 and 1 with hysteresis, we refer to the proposed logic-based algorithms as hybrid algorithms. 

The design of the logic and parameters of the individual algorithms is done using the Lyapunov functions
\begin{equation} \label{eqn:VfunctionHBF}
	V_{\xlogic}(\xp) := \gamma_{\xlogic} \left(L(\xp_1) - L^* \right) + \frac{1}{2} \left|\xp_2\right|^2
\end{equation}
defined for each $\xlogic \in \xlogicSpace$ and each $\xp \in \reals^{2n}$. As evidenced by \cref{def:Convexity} in \Cref{sec:Preliminaries}, the set of nonstrongly convex functions includes a subset of functions $L$ which have a connected continuum of minimizers, with the most extreme case being linear functions \cite{boyd2004convex} \cite{nocedal2006numerical}. Therefore, for nonstrongly convex functions\footnote{Since the value of $L$ is the same for all $\xp_1 \in \A_1$, $L(\A_1)$ is a singleton.}, $L^* := L(\A_1) \in \reals$ is its minimum value. 

{\color{red}
To define the closed set $\T_{0,1}$ and ensure Lipschitz continuity of the static state-feedback laws $\hcq$ in \cref{eqn:HBF_HCQ},  We impose the following assumption\footnote{In the case where $L$ is $\mathcal{C}^2$ and strongly convex, this implies there exists some $M > 0$ such that $\nabla L$ is Lipschitz continuous.} on $\nabla L$.
\begin{assumption}[Lipschitz Continuity of $\nabla L$] \label{ass:Lipschitz}
	the function $\nabla L$ is Lipschitz-continuous with constant $M > 0$, namely,
	\begin{enumerate}[label={(LC\arabic*)},leftmargin=*]
		\item \label{item:LC1} $\left|\nabla L(\xp_1) - \nabla L(u_1)\right| \leq M \left|\xp_1 - u_1\right|$;
		\item \label{item:LC2} $L(\xp_1) \leq L(u_1) + \left\langle \nabla L(u_1), \xp_1 - u_1 \right\rangle + \frac{M}{2}\left|\xp_1 - u_1\right|^2$.
	\end{enumerate}
	for all $\xp_1, u_1 \in \reals^n$.
\end{assumption}

Then, using \cref{def:Convexity}, the suboptimality condition in \cref{lemma:ConvexSuboptimality}, the Lyapunov functions in \cref{eqn:VfunctionHBF}, letting $\varepsilon_0 > 0$, $\alpha > 0$, $c_0 > 0$, and $\gamma_0 > 0$ from $\hczero$ be such that
\begin{subequations} \label{eqn:UTilde0SetEquations}
	\begin{align} 
		\tilde{c}_0 & := \varepsilon_0 \alpha > 0\label{eqn:UTilde0SetEquationsA}\\ 
		d_0 & := c_0 - \gamma_0 \left(\frac{\tilde{c}_0^2}{\alpha}\right) > 0. \label{eqn:UTilde0SetEquationsB}
	\end{align}
\end{subequations}
and letting $\varepsilon_{1,0} \in (0,\varepsilon_0)$, $\alpha > 0$, and $c_{1,0} \in (0, c_0)$ be such that
\begin{subequations} \label{eqn:TTilde10SetEquations}
	\begin{align}
		\tilde{c}_{1,0} & := \varepsilon_{1,0} \alpha \in (0, \tilde{c}_0) \label{eqn:TTilde10SetEquationsA}\\
		d_{1,0} & := 2c_{1,0} - 2\gamma_1 \left(\frac{\tilde{c}_{1,0}^2}{\alpha} \right) \in \left(0,d_0 \right) \label{eqn:HatD10}
	\end{align}
\end{subequations}
we define the sets $\U_0$ and $\T_{1,0}$ as in \cref{eqn:U0} and \cref{eqn:T10}, respectively. The parameters $\tilde{c}_0$, $d_0$, $\lambda_0$, and $\gamma_0$ are designed so that $\U_0$ is in the region where $\hczero$ is to be used. In this design, $\lambda_0$ is large to avoid oscillations when converging to the minimum. By construction, $\T_{1,0}$ is in the interior of $\U_0$.

Using \cref{ass:Lipschitz}, \cref{lemma:ConvexSuboptimality}, and choosing $\hat{c}_0 > c_0$, we define the set 
\begin{equation} \label{eqn:T01}
	\T_{0,1} \subset \defset{\xp \in \reals^{2n}}{\gamma_0 \left(\frac{\alpha}{M^2} \right) \left|\nabla L(\xp_1)\right|^2 + \frac{1}{2}\left|\xp_2\right|^2 \geq \hat{c}_0}.
\end{equation}
This set defines the (closed) complement of a sublevel set with level larger than $c_0$.  It is used for the design of the set $D_0$, which triggers the jumps from using $\hczero$ to using $\hcone$, so that when, in particular, the state $z_1$ is far from the set $\A_1$, then $\kappa_1$ is used to steer it back to nearby it. For details on the derivations of these sets, see \cref{sec:DerivOfSets}.

We can apply our main result from \Cref{sec:BasicProperties} to this special case as follows. \Cref{lemma:HBCC} and \cref{prop:ExistenceC} hold for the hybrid closed-loop algorithm $\HS$, defined via \cref{eqn:HS-TimeVarying}-\cref{eqn:CAndDGradientsNestNSC}, omitting the state $\tau$ and with static state-feedback $\hcq$ in \cref{eqn:HBF_HCQ}, since the following conditions are satisfied.
\begin{enumerate}
	\item Due to $L$ satisfying \cref{ass:LisNSCVX,ass:QuadraticGrowth,ass:Lipschitz}, the sets $\U_0$, $\T_{1,0}$, and $\T_{0,1}$, defined via \cref{eqn:U0}, \cref{eqn:T10}, and \cref{eqn:T01} are closed by construction. Therefore \cref{item:C1} of \cref{ass:AssumpsForHBC} also holds.
	\item Due to $L$ satisfying \cref{ass:Lipschitz}, \cref{item:C2} of \cref{ass:AssumpsForHBC} also holds for $\dot{x} = F(x)$.
\end{enumerate}
\Cref{thm:GASGen} holds due to the following additional conditions being satisfied.
\begin{enumerate}
	\item We impose \cref{ass:CompactAndConnected} on $\A_1$.
	\item The closed-loop algorithm $\HS_1$ in \cref{eqn:Hq}, resulting from $\hcone$ in \cref{eqn:HBF_HCQ}, has the set $\A_1 \times \{0\}$ uniformly globally asymptotically stable as stated in \cref{thm:GAS-HBF}. This is a stronger condition than that in \cref{item:UC1} of \cref{ass:UnitingControl}.
	\item The closed-loop algorithm $\HS_0$ in \cref{eqn:Hq}, resulting from $\hczero$ in \cref{eqn:HBF_HCQ}, has the set $\A_1 \times \{0\}$ globally asymptotically stable as stated in \cref{thm:GAS-HBF}. Therefore, \cref{item:UC3} of \cref{ass:UnitingControl} holds.
	\item The existence of the constants $\tilde{c}_{1,0} \in (0, \tilde{c}_0)$ and $d_{1,0} \in (0, d_0)$, defined via \cref{eqn:UTilde0SetEquations} and \cref{eqn:TTilde10SetEquations}, which, combined with the condition in \cref{eqn:V1Bound}, leads to every $\xp \in \T_{1,0}$ being in a $c_{1,0}$-sublevel set of $V_1$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality}, contained in the interior of $\U_0$, implies that there exist $\tilde{c}_1 \in (0,\tilde{c}_{1,0})$ and $d_1 \in (0,d_{1,0})$ such that \cref{eqn:c1d1Set} holds. Moreover, since \cref{item:UC3} holds, then each solution $\xp$ to $\HS_0$ with initial condition in $\T_{1,0}$, resulting from applying $\hczero$, remains in $\U_0$. Therefore, \cref{item:UC2} holds.
	\item The construction of $\U_0$ and $\T_{0,1}$, in \cref{eqn:U0} and \cref{eqn:T01}, respectively, with $\tilde{c}_0 > 0$ and $d_0 > 0$ defined via \cref{eqn:UTilde0SetEquations} and with $\hat{c}_0 > c_0 > 0$, satisfies \cref{item:UC4} of \cref{ass:UnitingControl}.	
%	the construction of $\U_0$ in \cref{eqn:U0}, with conditions in \cref{eqn:UTilde0SetEquations} and \cref{eqn:V0Bound} leading to every $\xp \in \U_0$ being in a $c_0$-sublevel set of $V_0$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality} and the construction of $\T_{0,1}$ in \cref{eqn:T01} as a closed complement of a sublevel set with level larger than $c_0$ such that $V_0$, defined via \cref{eqn:VfunctionHBF} is lower bounded via \cref{item:LC1} with $u_1 = \xp_1^*$ and \cref{eqn:QuadraticGrowth}, then \cref{item:UC4} of \cref{ass:UnitingControl} holds. 
\end{enumerate}}

%{\color{red}Since the ODE in \cref{eqn:HBF} is time-invariant, then the hybrid closed-loop system $\HS$ uses the simplified version of the framework, with state $x := (\xp,\xlogic) \in \reals^{2n} \times \xlogicSpace$ and data $(C,F,D,G)$ defined as follows:
%\begin{subequations} \label{eqn:HS-TimeInvariant}
%	\begin{align}
%		F(x) := & \matt{\matt{\xp_2\\ \kappa_{\xlogic}(\hp_{\xlogic}(\xp))}\\ 0} & \forall x \in C := C_0 \cup C_1\\
%		G(x) := & \matt{\xp\\1-\xlogic} & \forall x \in D := D_0 \cup D_1
%	\end{align}
%\end{subequations}  
%where $C_0$, $C_1$, $D_0$, and $D_1$ are defined as
%\begin{subequations} \label{eqn:CAndDGradients}
%	\begin{align}
%		&C_0 := \U_0 \times \{0\}, \ C_1 := \overline{\reals^{2n}\setminus \T_{1,0}} \times \{1\}\\
%		&D_0 := \T_{0,1} \times \{0\}, \ D_1 := \T_{1,0}\times \{1\}. 
%	\end{align}
%\end{subequations}}

%The sets $\U_0$, $\T_{1,0}$, and $\T_{0,1}$, defined via \cref{eqn:U0}, \cref{eqn:T10}, and \cref{eqn:T01}, respectively, are closed by construction. Moreover, the static state-feedback laws in \cref{eqn:HBF_HCQ} satisfy \cref{item:C2}, since by \cref{ass:Lipschitz} $\nabla L$ is Lipschitz continuous. Therefore, hybrid closed-loop system $\HS$ in \cref{eqn:HS-TimeVarying}, with $C$ and $D$ defined via \cref{eqn:CAndDGradientsNestNSC}, $\hcq$ defined in \cref{eqn:HBF_HCQ}, and $\U_0$, $\T_{1,0}$, and $\T_{0,1}$ defined via \cref{eqn:U0}, \cref{eqn:T10}, and \cref{eqn:T01}, is well-posed as it satisfies the hybrid basic conditions, as stated in \cref{lemma:HBCC}. When, additionally, the objective function $L$ satisfies \cref{ass:QuadraticGrowth}, every maximal solution to the hybrid closed-loop system $\HS$ is bounded and complete, as stated in \cref{prop:ExistenceC}.

% Here, we need to explain how this special case meets the assumptions needed for the general result to cover UGAS!
%{\color{red}The static state-feedback laws $\hcq$, defined via \cref{eqn:HBF_HCQ}, are such that $\A_1 \times \{0\}$ is uniformly globally asymptotically stable for $\HS_{\xlogic}$ as stated in \cref{thm:GAS-HBF}, satisfying \cref{item:UC1,item:UC3} of \cref{ass:UnitingControl}. The existence of the constants $\tilde{c}_{1,0} > 0$ and $d_{1,0} > 0$, defined via \cref{eqn:TTilde10SetEquations}, which, combined with the condition in \cref{eqn:V1Bound}, lead to  every $\xp \in \T_{1,0}$ being in a $c_{1,0}$-sublevel set of $V_1$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality}, imply that there exist $\tilde{c}_1 \in (0,\tilde{c}_{1,0})$ and $d_1 \in (0,d_{1,0})$ such that $\left(\A_1 + \tilde{c}_1 \ball \right) \times \left(\{0\} + d_1 \ball\right) \subset \T_{1,0}$, where $\T_{1,0}$ is defined via \cref{eqn:T10}. Moreover, due the the construction of $\U_0$ in \cref{eqn:U0}, with conditions in \cref{eqn:UTilde0SetEquations} and \cref{eqn:V0Bound} leading to every $\xp \in \U_0$ being in a $c_0$-sublevel set of $V_0$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality} and the construction of $\T_{0,1}$ in \cref{eqn:T01} as a closed complement of a sublevel set with level larger than $c_0$ such that $V_0$ is lower bounded via \cref{item:LC1} with $u_1 = \xp_1^*$ and \cref{eqn:QuadraticGrowth}, then the sets $\U_0$, $\T_{1,0}$, and $\T_{0,1}$ satisfy \cref{ass:UnitingControl}. Additionally, since $\A_1$ satisfies \cref{ass:CompactAndConnected}, then the hybrid closed-loop system $\HS$, resulting from $\hcq$ in \cref{eqn:HBF_HCQ}, has the set $\A$, defined via \cref{eqn:SetOfMinimizersHS-NSCVX}, uniformly globally asymptotically stable, as stated in \cref{thm:GASGen}.}

%Since the conditions in \cref{eqn:UTilde0SetEquations} and \cref{eqn:V0Bound} lead to every $\xp \in \U_0$ being in a $c_0$-sublevel set of $V_0$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality}, then \cref{item:S1} is satisfied. Since the conditions in \cref{eqn:TTilde10SetEquations} and \cref{eqn:V1Bound} lead to every $\xp \in \T_{1,0}$ being in a $c_{1,0}$-sublevel set of $V_1$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality}, then \cref{item:S2} is satisfied. Moreover, since $\T_{0,1}$ in \cref{eqn:T01} is a closed complement of a sublevel set with level larger than $c_0$ such that $V_0$ is lower bounded via \cref{item:LC1} with $u_1 = \xp_1^*$ and \cref{eqn:QuadraticGrowth}, then \cref{item:S3} is satisfied. When, in addition to this,  $\A_1$ satisfies \cref{ass:CompactAndConnected}, and since $\HS_{\xlogic}$ has the set $\A_1 \times 0$ uniformly globally asymptotically stable by \cref{thm:GAS-HBF} -- which is a stronger assumption than \cref{ass:UGAS}, then the hybrid closed-loop system $\HS$, resulting from $\hcq$ in \cref{eqn:HBF_HCQ}, has the set $\A$, defined via \cref{eqn:SetOfMinimizersHS-NSCVX}, uniformly globally asymptotically stable, as stated in \cref{thm:GASGen}.

{\color{red}Under \cref{ass:LisNSCVX,ass:QuadraticGrowth,ass:Lipschitz}, the hybrid closed-loop system $\HS$, resulting from $\hcq$ defined via \cref{eqn:HBF_HCQ} has a hybrid convergence rate that is exponential. To prove such a rate in the following theorem, we use \cref{thm:HBFConvergenceRate}.
	
% This will be the convergence rate proof. Take the material from below! 
\begin{theorem}[Convergence rate for $\HS$]
	Let $L$ satisfy \cref{ass:LisNSCVX,ass:QuadraticGrowth,ass:Lipschitz}. Additionally, let $\lambda_{\xlogic} > 0$, $\gamma_{\xlogic} > 0$, $\varepsilon_{1,0} \in (0,\varepsilon_0)$, $\alpha > 0$ from  \cref{ass:QuadraticGrowth}, $c_{1,0} \in (0, c_0)$, $\tilde{c}_{1,0} \in (0, \tilde{c}_0)$ in \cref{eqn:UTilde0SetEquationsA} and \cref{eqn:TTilde10SetEquationsA}, $d_{1,0} \in (0, d_0)$ in \cref{eqn:UTilde0SetEquationsB} and \cref{eqn:HatD10}, $\hat{c}_0 > c_0$, $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:T10}, and $\T_{0,1}$ in \cref{eqn:T01}. Then, each maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j),\xlogic(t,j))$ to the hybrid closed-loop system $\HS$ satisfies
	\begin{equation} \label{eqn:HBFHybridConvergenceRate}
		L(\xp_1(t,j) - L^*) \leq \left(L(\xp_1(0,0)) - L^*\right) \exp \left(-\frac{\psi}{2} t\right)
	\end{equation}
	for all $(t,j) \in \dom x$, where $\psi > 0$, $\psi - \lambda_{\xlogic} < 0$ comes from \cref{thm:HBFConvergenceRate}.
\end{theorem}

\begin{proof}
	To prove the exponential convergence bound in \cref{eqn:HBFHybridConvergenceRate}, since $L$ is nonstrongly convex and has quadratic growth away from $\A_1$, by \cref{ass:LisNSCVX,ass:QuadraticGrowth}, then by \cref{thm:HBFConvergenceRate} each maximal solution $t \mapsto (\xp_1(t),\xp_2(t))$ to the individual heavy ball algorithms $\HS_0$ and $\HS_1$ satisfy \cref{eqn:HBFHybridConvergenceRate} for all $t \geq 0$, where $\psi > 0$, $\psi - \lambda_{\xlogic} < 0$. Due to the construction of $G$, the state $\xp$ does not change in $D$. Moreover, due to the construction of $D$, in \cref{eqn:CAndDGradientsNestNSC}, with  $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:T10}, and $\T_{0,1}$ in \cref{eqn:T01}, with $\tilde{c}_{1,0} \in (0, \tilde{c}_0)$ in \cref{eqn:UTilde0SetEquationsA} and \cref{eqn:TTilde10SetEquationsA}, with $d_{1,0} \in (0, d_0)$ in \cref{eqn:UTilde0SetEquationsB} and \cref{eqn:HatD10}, and with $\hat{c}_0 > c_0$, as described in the proof of \cref{thm:GASGen} solutions to $\HS$ are guaranteed to jump no more than twice. Therefore, due to the construction of $G$ and $D$, and due to the convergence rates of $\HS_1$ and $\HS_0$, then each maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j),\xlogic(t,j))$ to the hybrid closed-loop system $\HS$ starting from $C_1$ satisfies \cref{eqn:HBFHybridConvergenceRate} for all $(t,j) \in \dom x$, where $\psi > 0$, $\psi - \lambda_{\xlogic} < 0$ comes from \cref{thm:HBFConvergenceRate}.
\end{proof}}

%The following result shows that the hybrid closed-loop system $\HS$, with $C$ and $D$ as defined via \cref{eqn:CAndDGradients}, has the set \cref{eqn:setOfMinimizersHS} globally asymptotically stable, with convergence that is exponential. To prove it, we use an invariance principle and \cref{thm:GAS-HBF,thm:HBFConvergenceRate}.
%\begin{theorem}[Uniform global asymptotic stability of $\A$ for $\HS$]
%	\label{thm:GASC}
%	Let $L$ satisfy \cref{ass:LisNSCVX,ass:QuadraticGrowth,ass:Lipschitz,ass:CompactAndConnected}. Additionally, let $\lambda_{\xlogic} > 0$, $\gamma_{\xlogic} > 0$, $\varepsilon_{1,0} \in (0,\varepsilon_0)$, $\alpha > 0$ from  \cref{ass:QuadraticGrowth}, $c_{1,0} \in (0, c_0)$, $\tilde{c}_{1,0} \in (0, \tilde{c}_0)$ in \cref{eqn:UTilde0SetEquationsA} and \cref{eqn:TTilde10SetEquationsA}, $d_{1,0} \in (0, d_0)$ in \cref{eqn:UTilde0SetEquationsB} and \cref{eqn:HatD10}, $\hat{c}_0 > c_0$, $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:T10}, and $\T_{0,1}$ in \cref{eqn:T01}. Then, the set $\A$ is uniformly globally asymptotically stable for $\HS$. Furthermore, each maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j),\xlogic(t,j))$ to the hybrid closed-loop system $\HS$ satisfies
%	\begin{equation} \label{eqn:HBFHybridConvergenceRate}
%		L(\xp_1(t,j) - L^*) \leq \left(L(\xp_1(0,0)) - L^*\right) \exp \left(-\frac{\psi}{2} t\right)
%	\end{equation}
%	for all $(t,j) \in \dom x$, where $\psi > 0$, $\psi - \lambda_{\xlogic} < 0$ comes from \cref{thm:HBFConvergenceRate}.
%\end{theorem}
%
%\begin{proof}
%	As shown in the proof of \cref{thm:GAS-HBF}, $\A_1 \times \{0\}$ is globally asymptotically stable for the individual heavy ball algorithms $\HS_{\xlogic}$. 
%	
%	Next, we address the global asymptotic stability of the hybrid closed-loop system $\HS$. By \cref{lemma:HBCC}, the hybrid closed-loop system $\HS$ meets the hybrid basic conditions.
%	Additionally, by \cref{lemma:ExistenceC}, every maximal solution $x$ to $\HS$ is bounded and complete. Moreover, by  \cref{ass:CompactAndConnected}, $\A_1$ is compact and connected. Therefore, by construction $\A$ is compact, and $\U = \reals^{2n}$ contains a nonzero open neighborhood of $\A$. 
%%	Furthermore, in the proof of Lemma \ref{lemma:ExistenceC}, the compactness of $W \subset \U = \reals^{2n}$, implies that $\U$ contains a nonzero open neighborhood of $\A$.
%	
%	For the hybrid closed-loop system $\HS$, a trajectory based approach will be used to prove the attractivity of $\A$. The types of trajectories possible for solutions are: 
%	\begin{enumerate}[label={\arabic*)},leftmargin=*]
%		\item Trajectories that start in $C_0$, namely, such that $\xp(0,0) \in \U_0$ and $\xlogic(0,0) = 0$;
%		\item Trajectories that start in the interior of $D_1$, namely, such that $\xlogic(0,0) = 1$ and either $\left|\nabla L(\xp_1(0,0))\right| < \tilde{c}_{1,0}$, $\frac{1}{2} \left|\xp_2(0,0)\right|^2 \leq d_{1,0}$ or $\left|\nabla L(\xp_1(0,0))\right| \leq \tilde{c}_{1,0}$, $\frac{1}{2} \left|\xp_2(0,0)\right|^2 < d_{1,0}$;
%		\item Trajectories that start on the boundary between $C_1$ and $D_1$, namely, such that $\left|\nabla L(\xp_1(0,0))\right| = \tilde{c}_{1,0}$, $\frac{1}{2}\left|\xp_2(0,0)\right|^2 = d_{1,0}$, and $\xlogic(0,0) = 1$;
%		\item Trajectories that start in the interior of $C_1$, namely, such that $\xlogic(0,0) = 1$ and either $\left|\nabla L(\xp_1(0,0))\right| > \tilde{c}_{1,0}$, $\frac{1}{2} \left|\xp_2(0,0)\right|^2 \geq d_{1,0}$ or $\left|\nabla L(\xp_1(0,0))\right| \geq \tilde{c}_{1,0}$, $\frac{1}{2} \left|\xp_2(0,0)\right|^2 > d_{1,0}$; 
%		\item Trajectories that start in $D_0$, namely, such that $\xp(0,0) \in \T_{0,1}$, defined via \cref{eqn:T01}, and $\xlogic(0,0) = 0$;
%	\end{enumerate}
%
%	Due to the construction of $\g$, the value of $\xp$ does not change during jumps. Furthermore, by the construction of $D$ with $\hat{c}_0 > c_0$, $c_0 > c_{1,0}$, $\tilde{c}_0 > \tilde{c}_{1,0}$, and $d_0 > d_{1,0}$, solutions that enter $D_0$ only jump once, and never enter $D_0$ again. This is also the case for $D_1$. Due to these same properties, solutions never jump directly from $D_0$ to $D_1$ or vice versa, but enter $C$ and flow before jumping again. Therefore, solutions to $\HS$ never have more than two jumps.
%
%	First we analyze trajectories of type 1). By \cref{ass:QuadraticGrowth}, $L$ satisfies \cref{eqn:QuadraticGrowth} for some $\alpha > 0$. Therefore, since $\tilde{c} > 0$ and $d_0 > 0$ are defined via \cref{eqn:UTilde0SetEquations}, then by \cref{lemma:ConvexSuboptimality}, when $\xp(0,0) \in \U_0$, it is in a $c_0$-sublevel set of $V_0$, as shown in \cref{eqn:V0c0SublevelSet}. Furthermore, since $\hat{c}_0 > c_0$ and since $\xlogic(0,0) = 0$, then $C_0$ does not share a boundary with $D_0$. Therefore, since $\dot{V}_0(\xp) \leq 0$ for each $\xp \in \reals^{2n}$, as shown in \cref{eqn:VdotHBF}, then all solutions starting in $C_0$ never jump, but instead only flow using $\hczero$. Therefore, the set $\A$ is attractive, for all trajectories of type 1).
%	
%	Next we analyze trajectories of type 2). When the state $\xp$ starts in the interior of $D_1$ the algorithm jumps, resetting $\xlogic$ to $0$ and assigning $u$ to $\hczero(\hp_0(\xp))$ while $\xp$ does not change. Then, the state $\xp$ is in $C_0$, and from such a point the solution follows the behavior of type 1) trajectories. Therefore, the set $\A$ is attractive, for all trajectories of type 2).
%	
%	Then, we analyze trajectories of type 3). Such a trajectory starts on the boundary between $C_1$ and $D_1$. For such initial conditions, $\dot{V}_1(\xp) = 0$ only when $\xp_2 = 0$ and $\dot{V}_1(\xp) < 0$ when $\xp_2 \neq 0$, as shown in \cref{eqn:VdotHBF}. Due to the way $C_1$ is defined, via \cref{eqn:CAndDGradients}, with $\T_{1,0}$ defined via \cref{eqn:T10}, the hybrid closed-loop algorithm can not flow from the initial state, since $V_1$ does not decrease when $\xp_2 = 0$ and since flowing would violate the definition of $C_1$ when $\xp_2 \neq 0$. Therefore, the hybrid closed-loop algorithm only jumps from the initial state, and from such a point the solution follows the behavior of type 2) trajectories. Therefore, the set $\A$ is attractive, for trajectories of type 3).
%	
%	Next, we analyze trajectories of type 4). When the state $\xp$ starts in the interior of $C_1$, the algorithm flows using $u = \hcone(\hp_1(\xp))$. Since $\dot{V}_1(\xp) \leq 0$ for each $\xp \in \reals^{2n}$, as shown in \cref{eqn:VdotHBF}, then the hybrid closed-loop algorithm flows until state $\xp$ reaches the boundary between $C_1$ and $D_1$. From such a point, the solution follows the behavior of type 3) trajectories. Therefore, the set $\A$ is attractive, for trajectories of type 4).
%	
%	Finally, we analyze trajectories of type 5). By \cref{ass:QuadraticGrowth}, $L$ satisfies \cref{eqn:QuadraticGrowth} for some $\alpha > 0$. Furthermore, $\nabla L$ is Lipschitz continuous with constant $M > 0$, by \cref{ass:Lipschitz}. Therefore, since $\hat{c}_0 > c_0$, then $D_0$ does not share a boundary with $C_0$. Consequently, when the state $\xp$ is in $D_0$, the hybrid closed-loop algorithm only jumps, resetting $\xlogic$ to $1$ and assigning $u$ to $\hcone(\hp_1(\xp))$ while $\xp$ remains the same. From such a point, the solution follows the behavior of type 4) trajectories. Therefore, the set $\A$ is attractive, for all trajectories of type 5). 
%	
%	% Also, needs more mention of the properties of the hybrid system that make that stable (?)
%	The behaviors for trajectories 1) through 5) are guaranteed by the following. The individual heavy ball algorithms $\HS_{\xlogic}$, for all $\xlogic \in \xlogicSpace$, were shown in the proof of \cref{thm:GAS-HBF} by \cref{eqn:VdotHBF} to be stable, for each $\xp \in \reals^{2n}$, since $\lambda_{\xlogic} > 0$ and $\gamma_{\xlogic} > 0$.
%	Additionally, the largest weakly invariant set for the individual heavy ball algorithms $\HS_{\xlogic}$ contained in \cref{eqn:LaSalleSetVHBF}, with $r = 0$, is equal to $\A_1 \times \{0\}$. Furthermore, by the suboptimality condition in \cref{lemma:ConvexSuboptimality} and by the construction of $\g$, $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:T10}, and $\T_{0,1}$ in \cref{eqn:T01}, once the state $\xp$ is inside $\T_{1,0}$, it will never reach the boundary of $\U_0$ when $\hczero$ is used. Due to these properties, and since every trajectory of the hybrid closed-loop algorithm $\HS$ ends with $\xlogic = 0$, every bounded and complete solution to $\HS$ converges to $\A$. Generally, the Lyapunov theorem and the invariance principle prove global pre-asymptotic stability. But since by \cref{lemma:ExistenceC} it was proved that every maximal solution is complete, then $\A$ is globally asymptotically stable. 
%	
%	Finally, to prove exponential convergence rate, since $L$ is nonstrongly convex and has quadratic growth away from $\A_1$, by \cref{ass:LisNSCVX,ass:QuadraticGrowth}, then by \cref{thm:HBFConvergenceRate} each maximal solution $t \mapsto (\xp_1(t),\xp_2(t))$ to the individual heavy ball algorithms $\HS_0$ and $\HS_1$ satisfy \cref{eqn:HBFHybridConvergenceRate} for all $t \geq 0$, where $\psi > 0$, $\psi - \lambda_{\xlogic} < 0$. Due to the construction of $G$, the state $\xp$ does not change in $D$. Moreover, due to the construction of $D$, in \cref{eqn:CAndDGradients}, solutions to $\HS$ are guaranteed to jump no more than twice. Therefore, due to the construction of $G$ and $D$, and due to the convergence rates of $\HS_1$ and
%	$\HS_0$, then each maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j),\xlogic(t,j))$ to the hybrid closed-loop system $\HS$ starting from $C_1$ satisfies \cref{eqn:HBFHybridConvergenceRate} for all $(t,j) \in \dom x$, where $\psi > 0$, $\psi - \lambda_{\xlogic} < 0$ comes from \cref{thm:HBFConvergenceRate}.
%\end{proof}

\begin{example} \label{ex:exampleHBF}
	
	\begin{figure}[thpb]
		\centering
		\setlength{\unitlength}{1.0pc}
		%		
		%		\vspace{-0.1cm}
		%
		\begin{picture}(30.8,12.1)(0,0)
			\footnotesize
%										
%					\put(0,0){\framebox(24,19)}
%										
			\put(0,0.5){\includegraphics[scale=0.4,trim={1.2cm 6cm 1.2cm 0.6cm},clip,width=30.8\unitlength]{Figures/HBFGradientsPlots.eps}}
			\put(0,6.2){$\xp_1$}
			\put(16,0){$t[s]$}
		\end{picture}
		\caption{A comparison of the evolution of $\xp_1$ over time for $\HS_0$, $\HS_1$, and $\HS$, defined via \cref{eqn:HS-TimeVarying} with $C$ and $D$ defined in \cref{eqn:CAndDGradientsNestNSC}, for a function $L(\xp_1) := \xp_1^2$ with a single minimizer at $\A_1 = \{0\}$. Heavy ball $\HS_1$ with $\lambda_1 = \frac{1}{5}$, shown in purple, settles to within $1\%$ of $\A_1$ in about 60.7 seconds. The heavy ball algorithm $\HS_0$ with $\lambda_0 = 30$, shown in green, settles to within $1\%$ of $\A_1$ in about 186.3 seconds.  The hybrid closed-loop system $\HS$, shown in blue, settles to within $1\%$ of $\A_1$ in about 2.9 seconds.}
		\label{fig:UnitingGradientsHBF}
	\end{figure}
	To show the effectiveness of the uniting algorithm, we compare it in simulation to the individual heavy ball algorithms $\HS_0$ and $\HS_1$. For this comparison, we use the objective function $L(\xp_1) := \xp_1^2$, with a single minimizer at $\A_1 = \{0\}$. For simulation, we used the heavy ball parameter values $\lambda_0 = 30$, $\lambda_1 = \frac{1}{5}$, and $\gamma_0 = \gamma_1 = \frac{1}{2}$. The parameter values for the uniting algorithm are $c_0 = 1200$, $c_{1,0} = 925$, $\varepsilon_0 = 12.5$, $\varepsilon_{1,0} = 6.3$, and $\alpha = 1$, which yield the values $\tilde{c}_0 = 12.5$, $\tilde{c}_{1,0} = 6.3$, $d_0 = 1.1219 \times 10^3$, and $d_{1,0} = 1810.31$, which are calculated via \cref{eqn:UTilde0SetEquations} and \cref{eqn:TTilde10SetEquations}. We also pick $\hat{c}_0 = c_0 + 1$. Initial conditions for $\HS_0$, $\HS_1$, and $\HS$ are $\xp_1(0,0) = -50$, $\xp_2(0,0) = 0$, and $\xlogic(0,0) = 0$.
	
	\Cref{fig:UnitingGradientsHBF} shows the $\xp_1$component over time for each of the algorithms\footnote{Code at \url{gitHub.com/HybridSystemsLab/UnitingGradientsHBF}}. Black dots with times labeled in seconds denote when each solution settles within $1\%$ of $\A_1$. Algorithm $\HS_1$, shown in purple, reaches the set $\A_1$ quickly with a rise time of about 2.9 seconds. However, it overshoots to about 36.4 at a peak time of 3.1 seconds. Then it continues oscillating until it settles within $1\%$ of $\A_1$ in about 60.7 seconds. Algorithm $\HS_0$, shown in green, slowly settles within $1\%$ of $\A_1$ in about 186.3 seconds, which is the same as its rise time. The hybrid closed-loop system $\HS$, shown in blue, settles within $1\%$ of $\A_1$ in about 2.9 seconds, which is also the same as its rise time. To show percent improvement of the uniting algorithm over the individual algorithms, we use the following formula:
	\begin{equation} \label{eqn:PercentImprovement}
		\left(\frac{\text{Time of other algorithm} - \text{Time of } \HS}{\text{Time of other algorithm}}\right) \times 100 \%
	\end{equation}
	Using this formula, the hybrid closed-loop algorithm shows a $95.3\%$ improvement over $\HS_1$ and a $98.5\%$ improvement over $\HS_0$.
\end{example}

\begin{example} \label{ex:exampleHBFNoise}
	To show that the uniform global asymptotic stability of $\A$, established in \cref{thm:GASGen}, is robust to small perturbations, we simulate the hybrid algorithm uniting local and global heavy ball algorithms, with zero-mean Gaussian noise added to measurements of the gradient. 
	
	The objective function $L$, heavy ball parameter values $\lambda_{\xlogic}$ and $\gamma_{\xlogic}$, uniting algorithm parameter values $c_0$, $c_{1,0}$, $\varepsilon_0$, $\varepsilon_{1,0}$, $\alpha$, $\tilde{c}_0$, $\tilde{c}_{1,0}$, $d_0$, $d_{1,0}$, and $\hat{c}_0$, and initial conditions $\xp_1(0,0)$, $\xp_2(0,0)$, and $\xlogic(0,0)$ are the same as those used in \cref{ex:exampleHBF}. However, noise is generated for trajectories of the perturbed system by drawing random values from the standard normal distribution with zero mean and standard deviations of $\sigma = 0.1$, $\sigma = 0.5$, and $\sigma = 1$, and interpolating intermediary values at intervals of $0.01$ between these random numbers, using \texttt{interp1} in MATLAB.
	
	\Cref{fig:HBFNoise} compares the trajectory of the nominal system with the three trajectories of the perturbed system. On the right hand side of \Cref{fig:HBFNoise}, a close-up of the local portion of the convergence is shown. The nominal system, which is shown in blue, converges to within $1\%$ of $\A_1$ in about $2.9$ seconds, as it does in \cref{fig:UnitingGradientsHBF}. The perturbed system with standard deviation of $\sigma = 0.1$, shown in purple, converges to  within $1\%$ of $\A_1$ in about $33.3$ seconds, due to a slightly earlier switch to $\hczero$, which was caused by the noise in measurements of the gradient. The perturbed systems with $\sigma = 0.5$ and $\sigma = 1$, shown in red and green, respectively, converge to within $1\%$ of $\A_1$ in about $1.71$ and $1.73$ seconds due to slightly later switches to $\hczero$.
	
	\begin{figure}[thpb]
		\centering
		\setlength{\unitlength}{1.0pc}
		\begin{picture}(30.8,14)(0,0)
			\footnotesize
%														
%									\put(0,0){\framebox(30.8,14)}
%														
			\put(0,0.5){\includegraphics[scale=0.4,trim={0.7cm 0.6cm 1cm 0.5cm},clip,width=30.8\unitlength]{Figures/HeavyBallGradientsNoise.eps}}
			\put(10,0){$\xp_1$}
			\put(25,0){$\xp_1$}
			\put(0,8){$\xp_2$}
		\end{picture}
		\caption{A comparison of the nominal and perturbed systems, with different values of $\sigma$. The nominal system, which converges to within a distance of $1\%$ of $\A_1$ in $2.9$ seconds, is in blue. The perturbed system with $\sigma = 0.1$, which converges to within $1\%$ of $\A_1$ in about $33.3$ seconds, is in purple. The perturbed system with $\sigma = 0.5$, which converges to within $1\%$ of $\A_1$ in about $1.71$ seconds, is in red. And the perturbed system with $\sigma = 1$, which converges to within $1\%$ of $\A_1$ in about $1.73$ seconds, is in green. Left: the full trajectory of each system. Right: a close up of the local convergence.}
		\label{fig:HBFNoise}
	\end{figure}
\end{example}

==> Sections/Nesterov-HBF.tex <==
The specific case, presented above, which unites Nesterov's algorithm globally and the heavy ball algorithm with large $\lambda$ locally, for nonstrongly convex $L$, has a global convergence rate of $\frac{1}{t + 2}$. We can make further improvements on the convergence rate when combining Nesterov's algorithm and the heavy ball algorithm for strongly convex $L$. With this in mind, we present a specific case of the framework in \Cref{sec:ModelingUF} which unites Nesterov's algorithm globally and the heavy ball algorithm with large $\lambda$ locally, for which the following assumption is satisfied:
\begin{assumption} \label{ass:LisCVX}
	$L$ is $\mathcal{C}^2$ and strongly convex. 
	%	That is, $L$ satisfies both Definitions \ref{def:StrongConvexity} and \ref{def:Convexity}. 
\end{assumption}
As with the specific case presented in \Cref{sec:NonstronglyConvexNest}, the specific case presented here exploits measurements of $\nabla L$.

%Since the ODE in \cref{eqn:MJODE} is time-invariant, then the hybrid closed-loop system $\HS$ uses the simplified version of the framework, with state $x := (\xp,\xlogic) \in \reals^{2n} \times \xlogicSpace$ and data $(C,F,D,G)$ defined via \cref{eqn:HS-TimeInvariant}. 

The static state-feedback law used for $\HS_0$ is defined in \cref{eqn:StaticStateFeedbackLawLocal} and the static state-feedback law used for $\HS_1$ is
\begin{equation} \label{eqn:StaticStateFeedbackLawGlobalSCVX}
		\hcone(\hp_1(\xp)) = -2d\xp_2 - \frac{1}{M_{\zeta}} \nabla L(\xp_1 + \beta \xp_2) 
\end{equation}
where $M_{\zeta} := M\zeta^2$, $\zeta > 0$, and $M >0$ is the Lipschitz constant for $\nabla L$. {\color{red}The state $\tau$ is not needed because the heavy ball algorithm in \cref{eqn:HBF} and Nesterov's algorithm in \cref{eqn:MJODE} are both time-invariant.} The local algorithm $\hczero$ corresponds to the heavy ball algorithm and the global algorithm $\hcone$ corresponds to Nesterov's algorithm. The output $\hp_0$ is defined via \cref{eqn:H0H1NSCNesterovHBF}, and the output $\hp_1$ is defined as
\begin{equation} \label{eqn:H1SCNesterov}
	\hp_1(\xp) := \matt{\xp_2\\ \nabla L(\xp_1 + \beta \xp_2)}.
\end{equation}
For strongly convex $L$, the constants $d$ and $\beta$ are typically chosen as follows
\begin{equation} \label{eqn:DandBeta}
	d := \frac{1}{(\sqrt{\kappa} + 1)}, \quad \beta := \frac{(\sqrt{\kappa} - 1)}{\sqrt{\kappa} + 1} 
\end{equation}
where $\kappa := \frac{M}{\mu} \geq 1$ is the condition number associated with $L$ \cite{boyd2004convex} \cite{nesterov2004introductory}. The constants in \cref{eqn:DandBeta} satisfy $2d + \beta = 1$. 

{\color{red}The Lyapunov function} $V_0$ {\color{red}is} defined via \cref{eqn:LyapunovHBF}, and the Lyapunov function $V_1$ {\color{red}is} defined as
\begin{equation} \label{eqn:LyapunovSCVXNesterov}
		V_1(\xp) := \frac{1}{2}\left|a(\xp_1 -\xp_1^*) + \xp_2\right|^2 + \frac{1}{M_{\zeta}} \left(L(\xp_1) - L^*\right) 
\end{equation}
where $L^* := L(\xp_1^*)$ and where $a>0$ is properly chosen.  

% Then explain the switching rules here!
Since quadratic growth is a weaker property
than strong convexity, even for $\mathcal{C}^1$ functions \cite{drusvyatskiy2018error} \cite{necoara2019linear}, then {\color{red}using the suboptimality condition in \cref{lemma:ConvexSuboptimality}, the Lyapunov functions in \cref{eqn:LyapunovHBF} and \cref{eqn:LyapunovSCVXNesterov}, letting $\varepsilon_0 > 0$, $\alpha > 0$, $c_0 > 0$, and $\gamma > 0$ from $\hczero$ in \cref{eqn:StaticStateFeedbackLawLocal} be such that $\tilde{c}_0$ is defined via \cref{eqn:UTilde0SetEquationsA} and $d_0$ is defined via \cref{eqn:d0Nest}, letting $\hat{c}_0 > c_0$, and letting $\varepsilon_{1,0} \in (0,\varepsilon_0)$, $\alpha > 0$, and $c_{1,0} \in (0, c_0)$ be such that 
\begin{equation} \label{eqn:TildeD10}
	d_{1,0} := c_{1,0} - a^2\left(\frac{\tilde{c}_{1,0}}{\alpha}\right)^2 - \frac{1}{M_{\zeta}}\left(\frac{\tilde{c}_{1,0}^2}{\alpha}\right) \in (0, d_0)
\end{equation}
where $\tilde{c}_{1,0}$ is defined in \cref{eqn:TTilde10SetEquationsA} and $d_0$ is defined in \cref{eqn:d0Nest}, we define the sets $\U_0$, $\T_{1,0}$, and $\T_{0,1}$ via \cref{eqn:U0}, \cref{eqn:T10}, and \cref{eqn:T01Nest}, respectively.

We can apply our main result from \Cref{sec:BasicProperties} to this special case as follows.
\Cref{lemma:HBCC} and \cref{prop:ExistenceC} hold for the hybrid closed-loop algorithm $\HS$ in \cref{eqn:HS-TimeVarying}-\cref{eqn:CAndDGradientsNestNSC}, omitting the state $\tau$ and with static state-feedback $\hczero$ in \cref{eqn:StaticStateFeedbackLawLocal} and $\hcone$ in \cref{eqn:StaticStateFeedbackLawGlobalSCVX}, since the following conditions are satisfied.
\begin{enumerate}
	\item Since $L$ satisfies \cref{ass:LisCVX}, this implies that $L$ also  satisfies\footnote{Quadratic growth is a weaker property than strong convexity \cite{drusvyatskiy2018error} \cite{necoara2019linear}} \cref{ass:QuadraticGrowth} and implies $\nabla L$ is Lipschitz continuous with constant $M > 0$. Hence, the sets $\U_0$, $\T_{1,0}$, and $\T_{0,1}$, defined via \cref{eqn:U0}, \cref{eqn:T10}, and \cref{eqn:T01Nest}. Therefore \cref{item:C1} of \cref{ass:AssumpsForHBC} also holds.
	\item Since $L$ satisfies \cref{ass:LisCVX}, implying $\nabla L$ is Lipschitz continuous with constant $M > 0$, then \cref{item:C2} of \cref{ass:AssumpsForHBC} also holds for $\dot{x} = F(x)$. 
\end{enumerate}
\Cref{thm:GASGen} holds due to the following additional conditions being satisfied.
\begin{enumerate}
	\item Since $L$ is strongly convex, $L$ has a single minimizer. Therefore $\A_1$ satisfies \cref{ass:CompactAndConnected}.
	\item The closed-loop algorithm $\HS_1$ in \cref{eqn:Hq}, resulting from $\hcone$ in \cref{eqn:StaticStateFeedbackLawGlobalSCVX}, has the set $\A_1 \times \{0\}$ uniformly globally asymptotically stable as stated in \cref{thm:GASNesterov}. This is a stronger condition than the condition in in \cref{item:UC1} of \cref{ass:UnitingControl}.
	\item The closed-loop algorithm $\HS_0$ in \cref{eqn:Hq}, resulting from $\hczero$ in \cref{eqn:StaticStateFeedbackLawLocal}, has the set $\A_1 \times \{0\}$ uniformly globally asymptotically stable, as stated in \cref{thm:GAS-HBF}. Therefore, \cref{item:UC3} of \cref{ass:UnitingControl} holds.
	\item The existence of the constants $\tilde{c}_{1,0} \in (0, \tilde{c}_0)$ and $d_{1,0} \in (0, d_0)$, defined via \cref{eqn:UTilde0SetEquationsA}, \cref{eqn:TTilde10SetEquationsA}, \cref{eqn:d0Nest}, and \cref{eqn:TildeD10}, which leads to every $\xp \in \T_{1,0}$ being in a $c_{1,0}$-sublevel set of $V_1$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality}, contained in the interior of $\U_0$, implies that there exist $\tilde{c}_1 \in (0,\tilde{c}_{1,0})$ and $d_1 \in (0,d_{1,0})$ such that \cref{eqn:c1d1Set} holds. Moreover, since \cref{item:UC3} holds, then each solution $\xp$ to $\HS_0$ with initial condition in $\T_{1,0}$, resulting from applying $\hczero$, remains in $\U_0$. Therefore, \cref{item:UC2} holds.
	\item The construction of $\U_0$ and $\T_{0,1}$, in \cref{eqn:U0} and \cref{eqn:T01Nest}, respectively, with $\tilde{c}_0 > 0$ and $d_0 > 0$ defined via \cref{eqn:UTilde0SetEquationsA} and \cref{eqn:d0Nest}, respectively, with $\hat{c}_0 > c_0 > 0$, satisfies \cref{item:UC4} of \cref{ass:UnitingControl}.
\end{enumerate}

% to construct the sets $C$ and $D$ in \cref{eqn:CAndDGradientsNestNSC}, we use $\U_0$ and $\T_{0,1}$, defined via \cref{eqn:U0} and \cref{eqn:T01Nest}, respectively, where $\varepsilon_0 > 0$, $\alpha > 0$, $c_0 > 0$, and $\gamma > 0$ from $\hczero$ are such that $\tilde{c}_0$ is defined via \cref{eqn:UTilde0SetEquationsA} and $d_0$ is defined via \cref{eqn:d0Nest}.

%To construct the set $\T_{1,0}$, let 
%Then, with $V_1$ given in \cref{eqn:LyapunovSCVXNesterov} and using \cref{def:Convexity} with $u_1 = \xp_1^*$, and \cref{lemma:ConvexSuboptimality}, we define $\T_{1,0}$ as {\color{red}in \cref{eqn:T10}}
%\begin{align} \label{eqn:c10SublevelSetNest}
%	V_1(\xp) & \leq  a^2\left|\xp_1\right|_{\A_1}^2 + \left|\xp_2\right|^2 + \frac{1}{M_{\zeta}} \left| \nabla L(\xp_1) \right| \left| \xp_1 \right|_{\A_1}.
%\end{align}
%Then, when $\left|\nabla L(\xp_1)\right| \leq \tilde{c}_{1,0}$, the suboptimality condition in \cref{lemma:ConvexSuboptimality} implies $\left|\xp_1\right|_{\A_1} \leq \frac{\tilde{c}_{1,0}}{\alpha}$, from where we get
%\begin{equation} \label{eqn:V1c10SublevelSet}
%	V_1(\xp) \leq a^2 \left(\frac{\tilde{c}_{1,0}}{\alpha}\right)^2 + \left|\xp_2\right|^2 + \frac{1}{M_{\zeta}} \left(\frac{\tilde{c}_{1,0}^2}{\alpha}\right). 
%\end{equation}
%Then, by defining
%\begin{equation} \label{eqn:TildeT10}
%	\T_{1,0} := \defset{\xp \in \reals^{2n}}{\left| \nabla L(\xp_1) \right| \leq \tilde{c}_{1,0}, \left|\xp_2\right|^2 \leq \tilde{d}_{1,0}}
%\end{equation}
%which, by construction, is contained in the interior of $\U_0$, defined in \cref{eqn:U0}. Then, every $\xp \in \T_{1,0}$ belongs to the $c_{1,0}$-sublevel set of $V_1$, defined via \cref{eqn:LyapunovSCVXNesterov}, namely, 
%%In fact, using the conditions in \cref{eqn:TTilde10SetEquationsA}, \cref{eqn:TildeD10}, and \cref{eqn:V1c10SublevelSet}, we have for each $\xp \in \T_{1,0}$,
%\begin{equation} \label{eqn:V1BoundSCNest}
%	V_1(\xp) \leq a^2 \left(\frac{\tilde{c}_{1,0}}{\alpha}\right)^2 + \left|\xp_2\right|^2 + \frac{1}{M_{\zeta}} \left(\frac{\tilde{c}_{1,0}^2}{\alpha}\right) \leq c_{1,0}.
%\end{equation}
%
%When $\xlogic = 1$, $\left| \nabla L(\xp_1) \right| \leq \tilde{c}_{1,0}$, and $\left|\xp_2\right|^2 \leq \hat{d}_{1,0}$, the supervisor will switch from the global algorithm $\hcone$ to the local algorithm $\hczero$.
%
%Employing $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:TildeT10}, and $\T_{0,1}$ in \cref{eqn:T01}, the flow and jump sets $C$ and $D$ are defined as follows:
%\begin{subequations} \label{eqn:CAndDGradientsNest}
%	\begin{align}
%		&C_0 := \U_0 \times \{0\}, \ C_1 := \overline{\reals^{2n}\setminus \T_{1,0}} \times \{1\}\\
%		&D_0 := \T_{0,1} \times \{0\}, \ D_1 := \T_{1,0}\times \{1\}.
%	\end{align}
%\end{subequations}

%Since $L$ satisfies \cref{ass:LisCVX}, this implies that $\nabla L$ is Lipschitz continuous with constant $M > 0$, and thus $\hczero$ and $\hcone$ defined via \cref{eqn:StaticStateFeedbackLawLocal} and \cref{eqn:StaticStateFeedbackLawGlobalSCVX}, respectively, satisfy \cref{item:C2}. Moreover, the sets $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:T10}, and $\T_{0,1}$ in \cref{eqn:T01Nest} are closed by construction. Therefore, hybrid closed-loop system $\HS$ in \cref{eqn:HS-TimeVarying}, with $C$ and $D$ defined via \cref{eqn:CAndDGradientsNestNSC}, is well-posed as it satisfies the hybrid basic conditions, as stated in \cref{lemma:HBCC}. Additionally, since the objective function $L$ satisfies \cref{ass:LisCVX}, this implies that $L$ also  satisfies\footnote{Quadratic growth is a weaker property than strong convexity \cite{drusvyatskiy2018error} \cite{necoara2019linear}} \cref{ass:QuadraticGrowth}. Therefore, every maximal solution to the hybrid closed-loop system $\HS$ in \cref{eqn:HS-TimeVarying}, with $C$ and $D$ defined via \cref{eqn:CAndDGradientsNestNSC}, is bounded and complete, as stated in \cref{prop:ExistenceC}.
%Additionally under \cref{ass:LisCVX}, every maximal solution $t \mapsto (\xp_1(0), \xp_2(0))$ of the closed loop algorithm $\HS_1$ is complete, bounded, and unique as stated in \cref{lemma:SCNesterovExistenceLemma}. Consequently, every
%maximal solution to $\HS$ is complete and bounded as stated in \cref{lemma:ExistenceC}. The proof follows quite similarly as the proof of \cref{lemma:ExistenceC}. 

%{\color{red}The static state-feedback laws $\hczero$ and $\hcone$, defined via \cref{eqn:StaticStateFeedbackLawLocal} and \cref{eqn:StaticStateFeedbackLawGlobalSCVX}, respectively, are such that $\A_1 \times \{0\}$ is uniformly globally asymptotically stable for $\HS_0$ and $\HS_1$, by \cref{thm:GAS-HBF} and \cref{thm:GASNesterov}, respectively, satisfying \cref{item:UC1,item:UC3} of \cref{ass:UnitingControl}. The existence of the constants $\tilde{c}_{1,0} > 0$ and $d_{1,0} > 0$, defined via \cref{eqn:TTilde10SetEquationsA} and \cref{eqn:TildeD10}, respectively, which, combined with the condition in \cref{eqn:V1BoundSCNest}, lead to every $\xp \in \T_{1,0}$ being in a $c_{1,0}$-sublevel set of $V_1$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality}, imply that there exist $\tilde{c}_1 \in (0,\tilde{c}_{1,0})$ and $d_1 \in (0,d_{1,0})$ such that $\left(\A_1 + \tilde{c}_1 \ball \right) \times \left(\{0\} + d_1 \ball\right) \subset \T_{1,0}$, where $\T_{1,0}$ is defined via \cref{eqn:T10}. Moreover, due the the construction of $\U_0$ in \cref{eqn:U0}, with conditions in \cref{eqn:UTilde0SetEquationsA}, \cref{eqn:d0Nest}, and \cref{eqn:V0Bound} leading to every $\xp \in \U_0$ being in a $c_0$-sublevel set of $V_0$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality} and the construction of $\T_{0,1}$ in \cref{eqn:T01Nest} as a closed complement of a sublevel set with level larger than $c_0$ such that $V_0$ is lower bounded via \cref{item:LC1} with $u_1 = \xp_1^*$ and \cref{eqn:QuadraticGrowth}, then the sets $\U_0$, $\T_{1,0}$, and $\T_{0,1}$ satisfy \cref{ass:UnitingControl}. Additionally, since $\A_1$ satisfies \cref{ass:CompactAndConnected}, then the hybrid closed-loop system $\HS$, resulting from $\hczero$ and $\hcone$ in \cref{eqn:StaticStateFeedbackLawLocal} and \cref{eqn:StaticStateFeedbackLawGlobalSCVX}, respectively, has the set $\A$, defined via \cref{eqn:SetOfMinimizersHS-NSCVX}, uniformly globally asymptotically stable, as stated in \cref{thm:GASGen}.

%{\color{red}Since the conditions in \cref{eqn:UTilde0SetEquationsA}, \cref{eqn:d0Nest}, and \cref{eqn:V0Bound} lead to every $\xp \in \U_0$ being in a $c_0$-sublevel set of $V_0$ via \cref{ass:LisCVX}, which is a stronger property than both \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality}, then \cref{item:S1} is satisfied. Additionally, since the conditions in \cref{eqn:TTilde10SetEquationsA}, \cref{eqn:TildeD10}, and \cref{eqn:V1Bound} lead to every $\xp \in \T_{1,0}$ being in a $c_{1,0}$-sublevel set of $V_1$ via \cref{def:Convexity} and \cref{lemma:ConvexSuboptimality}, then \cref{item:S2} is satisfied. Moreover, since $\T_{0,1}$ in \cref{eqn:T01} is a closed complement of sublevel set with level larger than $c_0$ such that $V_0$ is lower bounded via \cref{item:LC1} with $u_1 = \xp_1^*$ and \cref{eqn:QuadraticGrowth}, then \cref{item:S3} is satisfied. When, in addition, $\A_1$ satisfies \cref{ass:CompactAndConnected}, and since $\HS_1$ has the set $\A_1 \times 0$ uniformly globally asymptotically stable by \cref{thm:GASNesterov} and $\HS_0$ has the set $\A_1 \times 0$ uniformly globally asymptotically stable by \cref{thm:GAS-HBF} -- satisfying \cref{ass:UGAS}, then the hybrid closed-loop system $\HS$, resulting from $\hczero$ defined via \cref{eqn:StaticStateFeedbackLawLocal} and $\hcone$ defined in \cref{eqn:StaticStateFeedbackLawGlobalSCVX} has the set $\A$, defined via \cref{eqn:SetOfMinimizersHS-NSCVX}, uniformly globally asymptotically stable, as stated in \cref{thm:GASGen}. 

Under \cref{ass:LisCVX}, the hybrid closed-loop system $\HS$, resulting from $\hczero$ defined via \cref{eqn:StaticStateFeedbackLawLocal} and $\hcone$ defined in \cref{eqn:StaticStateFeedbackLawGlobalSCVX} has a hybrid convergence rate that is exponential. To prove it in the following theorem, we use \cref{prop:ConvRateSCL}.

\begin{theorem}
	Let $L$ satisfy \cref{ass:LisCVX}. Additionally, let $M_{\zeta} := M\zeta^2$, $\zeta > 0$, $M >0$, $\lambda > 0$, $\gamma > 0$, $\varepsilon_{1,0} \in (0, \varepsilon_0)$, $c_{1,0} \in (0,c_0)$, $c_0 > 0$, $\tilde{c}_{1,0} \in (0,\tilde{c}_0)$ from \cref{eqn:UTilde0SetEquationsA} and \cref{eqn:TTilde10SetEquationsA}, $d_{1,0} \in (0,d_0)$ from \cref{eqn:d0Nest} and \cref{eqn:TildeD10}, $\hat{c} > c_0$,  $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:T10}, and $\T_{0,1}$ in \cref{eqn:T01Nest}. Then, each maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j),\xp_2(t,j),\xlogic(t,j))$ of the hybrid closed-loop algorithm $\HS$ starting from $C_1$ satisfies, 
	%	for all $(t,j) \in \dom x$,
	\begin{equation} \label{eqn:UnitingConvergenceRateSC}
		L(\xp_1(t,0)) - L^* \leq (L(\xp_1(0,0)) - L^*)\exp(-a t)
	\end{equation}
	for each $t \in I^0$ where $q$ is equal to 1, and
	%	which $q$ is equal to 1 and 
	\begin{equation} \label{eqn:UnitingConvergenceRateSCHS0}
		L(\xp_1(t,1)) - L^* \leq (L(\xp_1(t_1,1)) - L^*)\exp(-2\mu t)
	\end{equation}
	for each $t \in I^1$ where $q$ is equal to 0, where $t_1$ is the time at which the first jump occurs, where $\mu > 0$, and where $a > 0$ is defined, for $\kappa := \frac{M}{\mu} \geq 1$, as\footnote{Note that, analogous to the case of $\bar{a}$ in Nesterov's algorithm for nonstrongly convex $L$, the constant $a$ can be upper bounded by 1 for all $\kappa \geq 1$ since when $\kappa = 1$, $a = 0$, and since as $\kappa \rightarrow \infty$, $a \rightarrow 1$.}
	\begin{equation} \label{eqn:ConstA}
		a := d + \frac{\beta}{2\kappa} = \frac{1}{\sqrt{\kappa}} - \frac{1}{2\kappa}
	\end{equation}
\end{theorem}

\begin{proof}
	By \cref{prop:ConvRateSCL}, each maximal solution $t \mapsto (\xp_1(t), \xp_2(t))$ to the global algorithm $\HS_1$ satisfies \cref{eqn:ConvergenceRateSCNesterov} for all $t \geq 0$, where $a > 0$ is defined via \eqref{eqn:ConstA}. By \cref{thm:HBFConvergenceRateSC}, each maximal solution $t \mapsto (\xp_1(t), \xp_2(t))$ to the local algorithm $\HS_0$ satisfies \cref{eqn:ExpDistToMin} for all $t \geq 0$, where $\mu > 0$. Due to the construction of $G$, defined via \cref{eqn:HS-TimeVarying}, the state $\xp$ does not change in $D$. Moreover, due to the construction of $D$, with $M_{\zeta} := M\zeta^2$, $\zeta > 0$, $M >0$, $\lambda > 0$, $\gamma > 0$, $\varepsilon_{1,0} \in (0, \varepsilon_0)$, $c_{1,0} \in (0,c_0)$, $c_0 > 0$, $\tilde{c}_{1,0} \in (0,\tilde{c}_0)$ from \cref{eqn:UTilde0SetEquationsA} and \cref{eqn:TTilde10SetEquationsA}, $d_{1,0} \in (0,d_0)$ from \cref{eqn:d0Nest} and \cref{eqn:TildeD10}, $\hat{c} > c_0$, $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:T10}, and $\T_{0,1}$ in \cref{eqn:T01Nest}, as described in the proof of \cref{thm:GASGen}, solutions to $\HS$ are guaranteed to jump no more than once when maximal solutions $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j),\xlogic(t,j))$ to $\HS$ start in $C_1$. Therefore, due to the construction of $G$ and $D$, and due to the convergence rates of $\HS_1$ and $\HS_0$, then each maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j),\xlogic(t,j))$ to the hybrid closed-loop algorithm $\HS$ that starts in $C_1$, satisfies \cref{eqn:UnitingConvergenceRateSC} for each $t \in I^0$ where $q$ is equal to 1, and \cref{eqn:UnitingConvergenceRateSCHS0} for each $t \in I^1$ where $q$ is equal to 0, where $t_1$ is the time at which the first jump occurs. This hybrid convergence rate holds for all $(t,j) \dom x$, with $a > 0$ defined in \cref{eqn:ConstA} and $\mu > 0$ from \cref{def:StrongConvexity}.
\end{proof}}

%% Then write a stability/convergence theorem and proof for this set of switching rules!
%The following corollary establishes that the hybrid closed-loop system $\HS$ with data defined in \cref{eqn:HS-TimeInvariant}, with $C$ and $D$ as in \cref{eqn:CAndDGradients}, has the set $\A$, defined via \cref{eqn:setOfMinimizersHS}, globally asymptotically stable, with a convergence rate that is exponential. To prove GAS and exponential convergence, we use an invariance principle, \cref{prop:ConvRateSCL}, \cref{lemma:ConvexSuboptimality}, and \cref{thm:HBFConvergenceRateSC,thm:GAS-HBF,thm:GAS-HBF}.
%
%\begin{corollary}[Uniform global asymptotic stability of $\A$ and convergence rate for $\HS$, when $L$ is strongly convex] \label{thm:GASNestQG}
%	Let $L$ satisfy \cref{ass:LisCVX}. Additionally, let $M_{\zeta} := M\zeta^2$, $\zeta > 0$, $M >0$, $\lambda > 0$, $\gamma > 0$, $\varepsilon_{1,0} \in (0, \varepsilon_0)$, $c_{1,0} \in (0,c_0)$, $c_0 > 0$, $\tilde{c}_{1,0} \in (0,\tilde{c}_0)$ from \cref{eqn:UTilde0SetEquationsA} and \cref{eqn:TTilde10SetEquationsA}, $d_{1,0} \in (0,d_0)$ from \cref{eqn:d0Nest} and \cref{eqn:TildeD10}, $\hat{c} > c_0$,  $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:T10}, and $\T_{0,1}$ in \cref{eqn:T01Nest}.
%	Then, the set $\A$, defined in \cref{eqn:setOfMinimizersHS}, is uniformly globally asymptotically stable for $\HS$ in \cref{eqn:HS-TimeInvariant}, with $C$ and $D$ as in \cref{eqn:CAndDGradients}. Furthermore, each maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j),\xp_2(t,j),\xlogic(t,j))$ of the hybrid closed-loop algorithm $\HS$ starting from $C_1$ satisfies, 
%	%	for all $(t,j) \in \dom x$,
%	\begin{equation} \label{eqn:UnitingConvergenceRateSC}
%		L(\xp_1(t,0)) - L^* \leq (L(\xp_1(0,0)) - L^*)\exp(-a t)
%	\end{equation}
%	for each $t \in I^0$ where $q$ is equal to 1, and
%	%	which $q$ is equal to 1 and 
%	\begin{equation} \label{eqn:UnitingConvergenceRateSCHS0}
%		L(\xp_1(t,1)) - L^* \leq (L(\xp_1(t_1,1)) - L^*)\exp(-2\mu t)
%	\end{equation}
%	for each $t \in I^1$ where $q$ is equal to 0, where $t_1$ is the time at which the first jump occurs, where $\mu > 0$, and where $a > 0$ is defined, for $\kappa := \frac{M}{\mu} \geq 1$, as\footnote{Note that, analogous to the case of $\bar{a}$ in Nesterov's algorithm for nonstrongly convex $L$, the constant $a$ can be upper bounded by 1 for all $\kappa \geq 1$ since when $\kappa = 1$, $a = 0$, and since as $\kappa \rightarrow \infty$, $a \rightarrow 1$.}
%	\begin{equation} \label{eqn:ConstA}
%		a := d + \frac{\beta}{2\kappa} = \frac{1}{\sqrt{\kappa}} - \frac{1}{2\kappa}
%	\end{equation}
%\end{corollary}
%
%\begin{proof}
%%	First we address the global asymptotic stability of the individual heavy ball ($\HS_0$) and Nesterov ($\HS_1$) algorithms. By \cref{thm:GAS-HBF}, $\A_1 \times \{0\}$ is globally asymptotically stable for the individual heavy ball algorithm $\HS_0$. Moreover, by \cref{thm:GASNesterov}, $\A_1 \times \{0\}$ is globally asymptotically stable for the individual Nesterov algorithm $\HS_1$.
%	By \cref{ass:LisCVX}, $L$ is strongly convex, which is a stronger condition than in \cref{ass:LisNSCVX}. Therefore, The hybrid closed-loop algorithm $\HS$ satisfies the hybrid basic conditions by \cref{lemma:HBCC} and every maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j), \xlogic(t,j))$ to $\HS$ is complete and bounded by \cref{lemma:ExistenceC}. By \cref{ass:LisCVX}, $L$ is strongly convex and therefore has a unique minimizer, which means the set $\A_1$, defined via \cref{eqn:setOfMinimizers} is compact. Therefore, by construction $\A$ is compact, and $\U = \reals^{2n}$ contains a nonzero open neighborhood of $\A$. This means the hybrid closed-loop algorithm $\HS$ satisfies the first and second assumptions of \cref{thm:hybrid Lyapunov theorem}.
%	
%	We use a trajectory based approach to prove the attractivity of $\A$, for the hybrid closed-loop algorithm $\HS$. The types of trajectories possible are the same as those listed in the proof of \cref{thm:UGAS_NSC}. Since $L$ is $\mathcal{C}^2$ and strongly convex by \cref{ass:LisCVX}, which is a stronger condition than in \cref{ass:LisNSCVX}, and since $\hat{c}_0 > c_0$, $c_0 > c_{1,0}$, $\tilde{c}_0 > \tilde{c}_{1,0}$, and $d_0 > d_{1,0}$, then by the construction of $\g$ and $D$, via \cref{eqn:HS-TimeInvariant} and \cref{eqn:CAndDGradients}, solutions to $\HS$ never have more than two jumps. 
%%	Due to the construction of $\g$, the value of $\xp$ does not change during jumps. Furthermore, by the construction of $D$ in \cref{eqn:CAndDGradients} with $\hat{c}_0 > c_0$, $c_0 > c_{1,0}$, $\tilde{c}_0 > \tilde{c}_{1,0}$, and $d_0 > \hat{d}_{1,0}$, solutions that enter $D_0$ only jump once, and never enter $D_0$ again. This is also the case for $D_1$. Due to these same properties, solutions never jump directly from $D_0$ to $D_1$ or vice versa, but enter $C$ and flow before jumping again. Therefore, solutions to $\HS$ never have more than two jumps.	
%%	
%%	
%%	First, trajectories of types 1) and 2) show the same behavior as the corresponding trajectory types in the the proof of Theorem \ref{thm:GASC}, and are described in detail therein. Therefore, the set $\A$ is attractive, for all trajectories of types 1) and 2).
%%	
%%	Next, we analyze trajectories of type 3). Such a trajectory starts on the boundary between $C_1$ and $D_1$. For such initial conditions, $\dot{V}_1(\xp) < 0$, as shown in \cref{eqn:StrongConvexityDotV}. Due to the way $C_1$ is defined, via \cref{eqn:CAndDGradients} with $\T_{1,0}$ defined in \cref{eqn:TildeT10}, the hybrid closed-loop algorithm can not flow from the initial state, since flowing would violate the definition of $C_1$. Therefore, the hybrid closed-loop algorithm only jumps from the initial state, and from such a point the solution follows the behavior of type 2) trajectories. Therefore, the set $\A$ is attractive, for all trajectories of type 3).
%%
%%	Next, we analyze trajectories of type 4). When the state $\xp$ starts in the interior of $C_1$, the algorithm flows using $u = \hcone(\hp_1(\xp))$. Since $\dot{V}_1(\xp) < 0$ for each $\xp \in \reals^{2n}$, as shown in \cref{eqn:StrongConvexityDotV}, then the hybrid closed-loop algorithm flows until state $\xp$ reaches the boundary between $C_1$ and $D_1$. From such a point, the solution follows the behavior of type 3) trajectories. Therefore, the set $\A$ is attractive, for trajectories of type 4).
%%	
%%	Finally, we analyze trajectories of type 5). By \cref{ass:LisCVX}, $L$ is $\mathcal{C}^2$ and strongly convex. This implies that $L$ also has quadratic growth away from $\A_1$ for some $\alpha > 0$, and that $\nabla L$ is Lipschitz continuous with constant $M > 0$. Therefore, since $\hat{c}_0 > c_0$, then $D_0$ does not share a boundary with $C_0$. Consequently, when the state $\xp$ is in $D_0$, the hybrid closed-loop algorithm only jumps, resetting $\xlogic$ to $1$ and assigning $u$ to $\hcone(\hp_1(\xp))$ while $\xp$ remains the same. From such a point, the solution follows the behavior of type 4) trajectories. Therefore, the set $\A$ is attractive, for all trajectories of type 5). 
%	Moreover, by the stronger condition in \cref {ass:LisCVX}, the attractivity of trajectories 1) through 5) are guaranteed by the following. The set $\A_1 \times \{0\}$ was shown in the proof of \cref{thm:GAS-HBF} by \cref{eqn:VdotHBF} to be stable, for the individual heavy ball algorithm $\HS_0$, since $\lambda > 0$ and $\gamma > 0$.
%	Additionally, the largest weakly invariant set for the individual heavy ball algorithm $\HS_0$ contained in \cref{eqn:LaSalleSetVHBF}, with $r = 0$, is equal to $\A_1 \times \{0\}$. Furthermore, the set $\A_1 \times \{0\}$ is globally asymptotically stable for $\HS_1$, by \cref{thm:GASNesterov}. Moreover, by the suboptimality condition in \cref{lemma:ConvexSuboptimality} and by the construction of $\g$, $\U_0$ in \cref{eqn:U0}, $\T_{1,0}$ in \cref{eqn:T10}, and $\T_{0,1}$ in \cref{eqn:T01Nest}, once the state $\xp$ is inside $\T_{1,0}$, it will never reach the boundary of $\U_0$ when $\hczero$ is used. Due to these properties, and since every trajectory of the hybrid closed-loop algorithm $\HS$ ends with $\xlogic = 0$, every bounded and complete solution to $\HS$ converges to $\A$. Generally, the Lyapunov theorem and the invariance principle prove uniform global pre-asymptotic stability. But since by \cref{lemma:ExistenceC} every maximal solution is complete, then $\A$ is uniformly globally asymptotically stable for $\HS$, with $C$ and $D$ defined via \cref{eqn:CAndDGradients}. 
%	
%	Finally, we prove the exponential convergence rate of the hybrid closed-loop system $\HS$. By \cref{prop:ConvRateSCL}, each maximal solution $t \mapsto (\xp_1(t), \xp_2(t))$ to the global algorithm $\HS_1$ satisfies \cref{eqn:ConvergenceRateSCNesterov} for all $t \geq 0$, where $a > 0$ is defined via \eqref{eqn:ConstA}. By \cref{thm:HBFConvergenceRateSC}, each maximal solution $t \mapsto (\xp_1(t), \xp_2(t))$ to the local algorithm $\HS_0$ satisfies \cref{eqn:ExpDistToMin} for all $t \geq 0$, where $\mu > 0$. Due to the construction of $G$, defined via \cref{eqn:HS-TimeInvariant}, the state $\xp$ does not change in $D$. Moreover, due to the construction of $D$, with $M_{\zeta} := M\zeta^2$, $\zeta > 0$, $M >0$, $\lambda > 0$, $\gamma > 0$, $\varepsilon_{1,0} \in (0, \varepsilon_0)$, $c_{1,0} \in (0,c_0)$, $c_0 > 0$, $\tilde{c}_{1,0} \in (0,\tilde{c}_0)$ from \cref{eqn:UTilde0SetEquationsA} and \cref{eqn:TTilde10SetEquationsA}, $d_{1,0} \in (0,d_0)$ from \cref{eqn:d0Nest} and \cref{eqn:TildeD10}, and $\hat{c} > c_0$, solutions to $\HS$ are guaranteed to jump no more than once when maximal solutions $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j),\xlogic(t,j))$ to $\HS$ start in $C_1$. Therefore, due to the construction of $G$ and $D$, and due to the convergence rates of $\HS_1$ and $\HS_0$, then each maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j),\xlogic(t,j))$ to the hybrid closed-loop algorithm $\HS$ that starts in $C_1$, satisfies \cref{eqn:UnitingConvergenceRateSC} for each $t \in I^0$ where $q$ is equal to 1, and \cref{eqn:UnitingConvergenceRateSCHS0} for each $t \in I^1$ where $q$ is equal to 0, where $t_1$ is the time at which the first jump occurs. This hybrid convergence rate holds for all $(t,j) \dom x$, with $a > 0$ defined in \cref{eqn:ConstA} and $\mu > 0$ from \cref{def:StrongConvexity}.
%\end{proof}

\begin{example} \label{ex:exampleSC}
		\begin{figure}[thpb]
		\centering
		\setlength{\unitlength}{1.0pc}
		%		
		%		\vspace{-0.1cm}
		%
		\begin{picture}(30.8,12.1)(0,0)
			\footnotesize
%													
%								\put(0,0){\framebox(30.8,12.1)}
%													
			\put(0,0.5){\includegraphics[scale=0.4,trim={1.2cm 5.3cm 1.2cm 0.5cm},clip,width=30.8\unitlength]{Figures/UnitingGradientsSCPlots.eps}}
			\put(0,6.1){$\xp_1$}
			\put(15.5,0.5){$t[s]$}
		\end{picture}
		\caption{A comparison of the evolution of $\xp_1$ over time for $\HS_0$, $\HS_1$, HAND-2, and $\HS$, defined via \cref{eqn:HS-TimeVarying} with $C$ and $D$ defined in \cref{eqn:CAndDGradientsNestNSC}, for a function $L(\xp_1) := \xp_1^2$ with a single minimizer at $\A_1 = \{0\}$. Nesterov's accelerated gradient descent ($\HS_1$), shown in purple, settles to within $1\%$ of $\A_1$ in about 9.1883 seconds. The heavy ball algorithm $\HS_0$, shown in green, settles to within $1\%$ of $\A_1$ in about 138.1 seconds. HAND-2, shown in orange, settles to within $1\%$ of $\A_1$ in about 1.3 seconds. The hybrid closed-loop system $\HS$, shown in blue, settles to within $1\%$ of $\A_1$ in about 0.7 seconds.}
		\label{fig:UnitingGradientsSC}
	\end{figure}

To show the effectiveness of the uniting algorithm, we compare it in simulation to the optimization algorithms $\HS_0$, $\HS_1$, and the HAND-2 algorithm from \cite{poveda2019inducing} for strongly convex functions $L$ satisfying Assumption \cref{ass:LisCVX}. Letting $\xp_1 := \xi$ and $\xp_2 := \xi + \frac{\tau}{2}\dot{\xi}$, the HAND-2 algorithm has state $(\xp, \tau) \in \reals^{2n+1}$ and data $(C,F,D,G)$ as in \cref{eqn:HANDFAndG}, with $c > 0$, $G_{\xp}(\xp,\tau) := [\xp_1^{\top} \xp_1^{\top}]^{\top}$,\\ $C := \defset{(\xp, \tau) \in \reals^{2n+1}}{\tau \in [T_{\min}, T_{\max}]}$, and $D := \defset{(\xp, \tau) \in \reals^{2n+1}}{\tau \geq T_{\max}}$, 
%$C$ and $D$ are
%\begin{subequations}
%	\begin{align}
%		C := & \defset{(\xp, \tau) \in \reals^{2n+1}}{\tau \in [T_{\min}, T_{\max}]}\\
%		D := & \defset{(\xp, \tau) \in \reals^{2n+1}}{\tau \geq T_{\max}}
%	\end{align}
%\end{subequations}
where $0 < T_{\min} < T_{\max} < \infty$. It is shown therein that each maximal solution $(t,j) \mapsto (\xp_1(t,j),\xp_2(t,j),\tau(t,j))$ of HAND-2 satisfies
\begin{equation} \label{eqn:PovedaNaBoundSC}
	L(\xp_1(t,j)) - L^* \leq k_a \left|\tilde{\xp}_1(0,0)\right|^2 \exp \left(-\tilde{k}_b \tilde{\alpha} \left(t + j\right)\right)
\end{equation}
for all $(t,j) \in \dom (\xp,\tau)$, where $k_a := 0.5 k_1 M$, $M > 0$, $k_1 := \frac{\left(c \mu \right)^{-1} + T^2_{\min}}{\Delta T^2}$, $\Delta T := T_{\max} - T_{\min}$, $0 < T_{\min} < T_{\max}$, $c > 0$, $\frac{1}{c \mu} < T^2_{\max} - T^2_{\min}$, $\tilde{k}_b := 1 - k_0$, $k_0\! :=\! \frac{\left(c \mu \right)^{-1} + T^2_{\min}}{T^2_{\max}}$, $j\! \geq \! \tilde{\alpha}(t+j)\! :=\! \frac{\max \{t+j - \Delta T, 0\}}{\Delta T + 1}$, and $\left|\tilde{\xp}_1(0,0)\right| := \left|\xp_1(0,0) - \xp_1^*\right|$. This bound holds when $\xp_1(0,0) = \xp_2(0,0)$ and $\tau(0,0) = T_{\min}$.

To compare these algorithms, we use the objective function  
%for this example 
$L(\xp_1) = \xp_1^2$, with a single minimizer at $\A_1 = \{0\}$. This objective function is strongly convex with $\mu = 2$ and its gradient is Lipschitz continuous with $M = 2$, which results in $\kappa = \frac{M}{\mu} = 1$. For simulation, we used the Nesterov parameter value $\zeta = 0.4$ and the heavy ball parameter values $\gamma = \frac{2}{3}$ and $\lambda = 40$. For HAND-2, we used the parameter values $T_{\max} = 4.3$, $T_{\min} = 3$, and $c = 0.78125$. The parameter values for the uniting algorithm are $c_0 = 20000$,  $c_{1,0} = 8700$, $\varepsilon_0 = 20$, $\varepsilon_{1,0} = 15$, and $\alpha = 1$, which yield the values $\tilde{c}_0 = 20$, $\tilde{c}_{1,0} = 15$, $d_0 = 1.9733 \times 10^4$, and $\tilde{d}_{1,0} = 7.9406 \times 10^3$, which are calculated via \cref{eqn:UTilde0SetEquationsA}, \cref{eqn:TTilde10SetEquationsA}, \cref{eqn:d0Nest}, and \eqref{eqn:TildeD10}. We also pick $\hat{c}_0 = c_0 + 1$. Initial conditions for $\HS_0$, $\HS_1$, and $\HS$ are $\xp_1(0,0) = 50$, $\xp_2(0,0) = 0$, and $\xlogic(0,0) = 1$, and for HAND-2 are $\xp_1(0,0) = 50$, $\xp_2(0,0) = 50$, and $\tau(0,0) = T_{\min}$.

\cref{fig:UnitingGradientsSC} shows the $\xp_1$ component over time for each of the algorithms\footnote{Code at \url{gitHub.com/HybridSystemsLab/UnitingGradientsNestSC}}. Black dots with times labeled in seconds denote when each solution settles within $1\%$ of $\A_1$. Algorithm $\HS_1$, shown in purple, reaches the set $\A_1$ quickly with a rise time of about 0.7 seconds. However, it overshoots to about -26.3, at a peak time of 1.27 seconds. Then it continues oscillating until it settles within $1\%$ of $\A_1$ in about 9.2 seconds. Algorithm $\HS_0$, shown in green, slowly settles within $1\%$ of $\A_1$ in about 138.1 seconds, which is the same as its rise time. The HAND-2 algorithm, shown in orange, settles to within $1\%$ of $\A_1$ in about 1.3 seconds. The hybrid closed-loop system $\HS$, shown in blue, settles within $1\%$ of $\A_1$ in about 0.7 seconds, which is also the same as its rise time. Using the formula in \cref{eqn:PercentImprovement}, this is a $43.4\%$ improvement over HAND-2, a $92.0\%$ improvement over $\HS_1$ and a $99.47\%$ improvement over $\HS_0$. 

% Paragraph here, about the comparisons.
\cref{fig:TrajectoriesPlots} compares different trajectories for $\HS$ and HAND-2, from different positive and negative values of $\left|\xp_1(0,0)\right|$, for the objective function $L(\xp_1) := \xp_1^2$. \cref{table:PercentImprovement} lists the times for which each trajectory settles to within $1\%$ of $\A_1$ for both $\HS$ and HAND-2, and shows the percent improvement of $\HS$ over HAND-2. All parameters for  $\HS$ and HAND-2 are the same as those used in \cref{fig:UnitingGradientsSC}, except that $\hat{c}_0 = 40001$ and $c_0 = 40000$ are used for all trajectories, the latter of which yields the parameter value $d_0 = 3.5733 \times 10^4$, calculated via \cref{eqn:d0Nest}. Furthermore, different $c_{1,0}$ are used for each trajectory -- listed in \cref{table:PercentImprovement} -- which leads to different values of $d_{1,0}$, calculated via \cref{eqn:TildeD10}, for each trajectory. The initial conditions $\xp_2(0,0) = 0$ and $\xlogic(0,0) = 1$ are used for all trajectories of $\HS$, and the initial conditions $\tau(0,0) = T_{\min}$ and $\xp_2(0,0) =\xp_1(0,0)$ are used for all trajectories of HAND-2. As can be seen in \cref{fig:TrajectoriesPlots} and in \cref{table:PercentImprovement}, the percent improvement of $\HS$ over HAND-2 ranges from $44.2\%$ to $42.4\%$, which shows consistency in the performance of $\HS$ versus HAND-2.

\begin{figure}[thpb]
	\centering
	\setlength{\unitlength}{1.0pc}
	%		
	%		\vspace{-0.1cm}
	%
	\begin{picture}(30.8,15.7)(0,0)
		\footnotesize
%												
%							\put(0,0){\framebox(30.8,15.7)}
%												
		\put(0,0.5){\includegraphics[scale=0.4,trim={1.2cm 0.1cm 1cm 0.5cm},clip,width=30.8\unitlength]{Figures/TrajectoriesPlots.eps}}
		\put(0,8.7){$\xp_1$}
		\put(7.7,0.5){$t[s]$}
		\put(23.2,0.5){$t[s]$}
	\end{picture}
	\caption{The evolution of $\xp_1$ over time, from different initial conditions, for $\HS$ and HAND-2. All trajectories are for the objective function $L(\xp_1) := \xp_1^2$, and the same parameters are used for HAND-2 and $\HS$ as in \cref{fig:UnitingGradientsSC}, except for $\hat{c}_0 = 40001$ and $c_0 = 40000$ for all trajectories, leading to $d_0 = 3.5733 \times 10^4$, and different values of $c_{1,0}$, listed in \cref{table:PercentImprovement}, leading to different values of $d_{1,0}$, calculated via \cref{eqn:TildeD10}.}
	\label{fig:TrajectoriesPlots}
\end{figure}

\begin{table}[thpb]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
	\hline
	 & & \multicolumn{2}{c|}{Time (s)} & $\%$ \\
	\cline{3-4} 
	 $\left|\xp_1(0,0)\right|$ & $c_{1,0}$ & $\HS$  & HAND-2  & Improvement  \\
	\hline
	\hline
	$110$ & $39000$ & 0.7285 & 1.3 & 44.0 \\
	\hline
	$100$ & $32500$ & 0.7345& 1.3 & 43.5 \\
	\hline
	$90$ & $26500$ & 0.7366 & 1.3 & 43.3 \\
	\hline
	$80$ & $21000$ & 0.7294 & 1.3 & 43.9 \\
	\hline
	$70$ & $16400$ & 0.7508 & 1.3 & 42.2 \\
	\hline
	$60$ & $12100$ & 0.7261 & 1.3 & 44.1 \\
	\hline
	$50$ & $8700$ & 0.7356 & 1.3 & 43.4 \\
	\hline
	$40$ & $5800$ & 0.7252 & 1.3 & 44.2 \\
	\hline
	$30$ & $3600$ & 0.7272 & 1.3 & 44.1 \\
	\hline
	$20$ & $2020$ & 0.7260 & 1.3 & 44.2 \\
	\hline
\end{tabular}
\caption{Times for which $\HS$ and HAND-2 settle to within $1\%$ of $\A_1$, and percent improvement of $\HS$ over HAND-2, for trajectories from different initial conditions, shown in \cref{fig:TrajectoriesPlots}. The objective function used for this plot is $L(\xp_1) := \xp_1^2$.}
\label{table:PercentImprovement}
\end{center}
\end{table}


As was stated in \cref{ex:exampleNSC}, the different choice of initial conditions between HAND-2 and $\HS$ is essential to the improved performance of the hybrid closed-loop algorithm $\HS$ over HAND-2. Namely, the bound in \cref{eqn:PovedaNaBoundSC} is guaranteed only when $\xp_1(0,0) = \xp_2(0,0)$. This means that the initial velocity for HAND-2 will be nonzero, unless the state starts at the set of minimizers, which can lead to overshoot in the transients of solutions. In comparison, $\xp_2(0,0)$ can be set to zero for $\HS$, which helps to avoid overshoot. Such overshoot in HAND-2 means this algorithm reaches the set of minimizers later than $\HS$, as seen in \cref{fig:UnitingGradientsSC}. 
%The choice of $\zeta$ is also important to the improved performance of $\HS$ over HAND-2, as HAND-2 is derived from the ODE for Nesterov's algorithm seen in \cite{su2014differential,wilson2016lyapunov,WibisonoE7351,krichene2015accelerated,poveda2019inducing}, namely, 
%\begin{equation} \label{eqn:SuNesterovODE}
%	\ddot{\xi} + \frac{\ell(p)}{t}\dot{\xi} + pct^{p-2}\nabla L(\xi) = 0
%\end{equation}
%which is shown in \cite{su2014differential} to be the limiting continuous-time system obtained from Nesterov's algorithm when $\ell(p) = p + 1$, $c = \frac{1}{p^2}$, and $p = 2$. Notice that this version of the ODE for Nesterov's algorithm does not have the parameter $\zeta$, and therefore time is not scaled for solutions to \eqref{eqn:HANDFAndG}.

% Look at more trajectories, and present information here! 
\end{example}

==> Sections/OtherGradAlgos.tex <==
\subsection{Uniting Other Gradient Algorithms}

In \Cref{sec:HBF-HBF,sec:NonstronglyConvexNest}, we illustrated the framework in \Cref{sec:ModelingUF} using specific cases involving different combinations of the heavy ball algorithm and Nesterov's algorithm, for $\hczero$ and $\hcone$. Other gradient-based algorithms, however, could be used as $\hczero$ and $\hcone$ for the general framework. One example includes classic gradient descent, which has the ODE
\begin{equation}
	\dot{\xi} + \gamma \nabla L(\xi) = 0
\end{equation}
where $\gamma > 0$ is tunable, and which is commonly known to have a convergence rate of $\frac{1}{t}$. As gradient descent does not have a ``velocity'' term, it tends to converge slowly, without oscillations near the minimizer -- similar behavior as seen for heavy ball with large $\lambda$. Due to this behavior, gradient descent could be used as the local algorithm $\hczero$ in the general framework in \Cref{sec:ModelingUF}, with either heavy ball with small $\lambda$ or Nesterov's algorithm as $\hcone$.

Another example includes the triple momentum method. The triple momentum method was first proposed in \cite{van2017fastest} as a discrete-time accelerated gradient method. A characterization of the continuous-time, high-resolution dynamical system, derived in \cite{sun2020high}, is
\begin{subequations} \label{eqn:TMODE}
	\begin{align}
		& \ddot{\xi} + 2\sqrt{\eta \left(\gamma,\lambda \right)}\dot{\xi} + \left(1+\sqrt{\eta\left(\gamma,\lambda \right) \gamma}\right) \nabla L(w) = 0\\
		& w := \xi + \sqrt{\gamma}\sigma \dot{\xi}\\
		& y := \xi + \sqrt{\gamma}\delta \dot{\xi}
	\end{align}
\end{subequations}
where $y \in \reals^n$ is the output, where the gradient is applied to $w \in \reals^n$, where $\gamma > 0$, $\lambda > 0$, $\sigma > 0$, and $\delta > 0$ are tunable parameters, and where $\eta(\gamma, \lambda)$ is
\begin{equation}
	\eta(\gamma, \lambda) := \left(\frac{1-\lambda}{\sqrt{\gamma}\left(1+\lambda \right)}\right)^2 \in (0,M].
\end{equation}
where $M > 0$ is the Lipschitz constant of $\nabla L$.
The authors in \cite{van2017fastest} and \cite{sun2020high} also give an ideal tuning of of the parameters as follows: 
\begin{equation} \label{eqn:IdealTMTuning}
	\left(\gamma,\lambda,\sigma,\delta \right) := \left(\frac{1+\rho}{M}, \frac{\rho^2}{2-\rho}, \frac{\rho^2}{\left(1+\rho\right)\left(2-\rho\right)}, \frac{\rho^2}{1-\rho^2}\right)
\end{equation}
where
\begin{equation}
	\rho := 1 - \frac{1}{\kappa}
\end{equation}
where $\kappa := \frac{M}{\mu}$, $\mu > 0$, is the condition number of $L$. The authors in \cite{sun2020high} characterize the convergence rate for \cref{eqn:TMODE} to be exponential, both for the general parameters and for the optimal tuning in \cref{eqn:IdealTMTuning}, and numerically found \cref{eqn:TMODE} to converge more quickly than Nesterov's algorithm, for given values of the condition number $\kappa$. Since \cref{eqn:TMODE} has an exponential convergence rate, it would be ideal for use as the global optimization algorithm $\hcone$ in the general framework, defined in \cref{sec:ModelingUF}, with either gradient descent or heavy ball with large $\lambda$ as $\hczero$.

==> Sections/Preliminaries.tex <==
\section{Preliminaries}
\label{sec:Preliminaries}

%\subsection{Hybrid Systems}

   

%The following definitions, from \cite{65} and \cite{220}, will be used in the analysis of the hybrid closed-loop system, obtained with the proposed hybrid control algorithm. 
%	\IfConf{\begin{defn}[Hybrid basic conditions]}{\begin{definition}[Hybrid basic conditions]} \label{def:HBCs} A hybrid system $\HS$ is said to satisfy the hybrid basic conditions if its data $(C,F,D,G)$ is such that
%		\begin{enumerate}[label={(A\arabic*)},leftmargin=*]
%			\item $C$ and $D$ are closed subsets of $\reals^n$;
%			\item $F : \reals^n \rightrightarrows \reals^n$ is outer semicontinuous and locally bounded relative to $C$, $C \subset \mathrm{dom} \ F$, and $F(x)$ is convex for every $x \in C$; 
%			\item \label{item:A3} $G : \reals^n \rightrightarrows \reals^n$ is outer semicontinuous and locally bounded relative to $D$, and $D \subset \mathrm{dom} \ G$.
%		\end{enumerate}
%	\IfConf{\end{defn}}{\end{definition}}
%The notions of stability, uniform global stability, pre-attractivity, uniform global pre-attractivity, and uniform global pre-asymptotic stability (UGpAS) are listed in the following definition, from \cite{220} and \cite{65}.
%\IfConf{\begin{defn}[Stability and attractivity notions]}{\begin{definition}[Stability and attractivity notions]} \label{def:UGpAS}
%	Given a hybrid \IfConf{closed-loop}{\\closed-loop} system $\HS$ as in \eqref{eqn:GeneralH}, a nonempty set $\mathcal{A} \subset \reals^n$ is said to be 
%	\begin{itemize}
%		\item \underline{Stable} for $\HS$ if for each $\eps > 0$ there exists $\delta > 0$ such that each solution $x$ to $\HS$ with $\left|x(0,0)\right|_{\mathcal{A}} \leq \delta$ satisfies $\left|x(t,j)\right|_{\mathcal{A}} \leq \eps$ for all $(t,j) \in \dom x$;
%		\item \underline{Uniformly globally stable} for $\HS$ if there exists a class-$\mathcal{K}_{\infty}$ function $\alpha$ such that any solution $x$ to $\HS$ satisfies $\left|x(t,j)\right|_{\mathcal{A}} \leq \alpha\left(\left|x(0,0)\right|_{\mathcal{A}}\right)$ for all $(t,j) \in \dom x$;
%		\item \underline{Pre-attractive} for $\HS$ if there exists $\mu > 0$ such that every solution $x$ to $\HS$ with $\left|x(0,0)\right|_{\mathcal{A}} \leq \mu$ is such that $(t,j) \mapsto \left|x(t,j)\right|_{\mathcal{A}}$ is bounded and if $x$ is complete then $\lim\limits_{(t,j) \in \dom x, \ t+j \rightarrow \infty} \left|x(t,j)\right|_{\mathcal{A}} = 0$;
%		%			\item \underline{Attractive} for $\HS$ if {\color{red}it is pre-attractive and} there exists $\mu > 0$ such that every maximal {\color{red}solution to} $\HS$ with {\color{red}$\left|x(0,0)\right|_{\A} \leq \mu$ is complete;}
%		%			\item \underline{Pre-Asymptotically stable} for $\HS$ if it is stable and pre-attractive.
%		%			\item \underline{Asymptotically stable} for $\HS$ if it is stable and attractive. 
%		\item \underline{Uniformly globally pre-attractive} for $\HS$ if for each $\eps > 0$ and $\delta > 0$ there exists $T > 0$ such that, for any solution $x$ to $\HS$ with $\left|x(0,0)\right|_{\mathcal{A}} \leq \delta$, $(t,j) \in \dom x$ and $t + j \leq T$ imply $\left|x(t,j)\right|_{\mathcal{A}} \leq \eps$;
%		\item \underline{Uniformly globally pre-asymptotically stable (UGpAS)} for $\HS$ if it is both\\ uniformly globally stable and uniformly globally pre-attractive.
%	\end{itemize}	
%\IfConf{\end{defn}}{\end{definition}}
%
%In the notions involving convergence in Definition \ref{def:UGpAS}, when every maximal solution is complete, then the prefix ``pre'' is dropped to obtain attractivity, uniform global attractivity (UGA), and uniform global asymptotic stability (UGAS). 
%The prefix ``pre'' is in the notions involving convergence in Definition \ref{def:UGpAS} to allow for maximal solutions that are not complete. When every maximal solution is complete, such a property guarantees that nontrivial solutions exist from each initial point in $C \cup D$ to the hybrid system resulting from using our proposed uniting algorithm.
%
%As was mentioned in Section \ref{sec:Background}, establishing UGAS for Nesterov's algorithm is a difficult problem to solve, due to its time-varying nature, as some solutions converge in a non-uniform way. We show in Section \ref{sec:ProofMainResult} that our proposed uniting algorithm overcomes such a difficulty. \IfConf{
%
%\vspace{-0.1cm}
%
%}{}

==> Sections/Suboptimality.tex <==
\section{Results on Suboptimality}
\label{sec:Suboptimality}



==> Sections/UnitingFramework.tex <==
\section{Problem Statement and General Uniting Framework} 
\label{sec:ProblemStatement}

\subsection{Problem Statement}
As illustrated in \cref{fig:MotivationalPlotTR}, the performance of Nesterov's accelerated gradient descent commonly suffers from oscillations near the minimizer. This is also the case for the heavy ball method when $\lambda > 0$ is small. However, when $\lambda$ is large, the heavy ball method converges slowly, albeit without oscillations. In \Cref{sec:Intro} we discussed how the heavy ball algorithm guarantees an exponential rate for strongly convex $L$ and a rate of $\frac{1}{t}$ for nonstrongly convex $L$, although it was demonstrated in \cite{sebbouh2019nesterov} that the heavy ball algorithm converges exponentially for nonstrongly convex $L$ when such an objective function also has the property of quadratic growth away from its minimizer.  We also discussed how Nesterov's algorithm guarantees an exponential convergence rate for strongly convex $L$ and a rate of $\frac{1}{t^2}$ for nonstrongly convex $L$. We desire to attain such rates, while avoiding oscillations via the heavy ball algorithm with large $\lambda$. We state the following general problem to solve as follows:

\begin{problem}\label{problem:ProbStatement}
	Given a scalar, real-valued, continuously differentiable objective function $L$ with a set of minimizers that is a singleton or a connected continuum set, and given two optimization algorithms $\hczero$ and $\hcone$, with $\hczero$ to be used locally and $\hcone$ to be used globally, design a uniting optimization framework that preserves the convergence rates of $\hczero$ and $\hcone$, without oscillations and with uniformity with respect to the compact sets of initial conditions, without knowing the function $L$ or the location of its minimizer, and with robustness to arbitrarily small noise in measurements of $\nabla L$.
\end{problem}

In this paper, we propose a framework for logic-based algorithms, which unite any two continuous-time, gradient-based optimization algorithms $\hczero$ and $\hcone$ to solve \cref{problem:ProbStatement}. The central idea is that the global optimization algorithm $\hcone$ provides fast convergence to the neighborhood of the set of minimizers and the local optimization algorithm $\hczero$ provides stable convergence in the neigborhood of the set of minimizers, without oscillations. A logic variable is used to indicate which algorithm -- either $\hczero$ or $\hcone$ -- is currently in use, and the switch between local and global algorithms is based on sublevel sets of the Lyapunov functions of $\hczero$ and $\hcone$. 
% Insert outline (in paragraph form) of this framework.
One difficulty in designing such a uniting framework is that the objective function $L$ and the set of minimizers are unknown, so the algorithm must be able to detect when to switch, and do so in a way that avoids chattering.

\subsection{Modeling of the Uniting Framework}
\label{sec:ModelingUF}
% Describe the general framework in much more general terms... don't have to define things like $\kappa_{\xlogic}$ until later! 
We interpret the ODEs in \cref{eqn:MJODE}, \cref{eqn:MJODENCVX}, and \cref{eqn:HBF} as control systems consisting of a plant and a control algorithm \cite{191} \cite{220}.  Then, defining $\xp_1$ as $\xi$ and $\xp_2$ as $\dot{\xi}$, the plant for these ODEs is given by 
the double integrator
\begin{equation}\label{eqn:HBFplant-dynamicsTR}
	\matt{\dot{\xp}_1\\ \dot{\xp}_2\\} = \matt{\xp_2\\ \up} =: \fp(\xp,u) \qquad (\xp,\up) \in \reals^{2n} \times \reals^n =: \Cp
\end{equation}
{\color{red}With this model, the class of optimization algorithms that we consider assign $u$ to a function of the state that involves the cost function, and such a function of the state may be time dependent. For instance, if the ODE in \cref{eqn:MJODE} is used, we have $u = \hc(\hp(\xp)) = -2d\xp_2 - \frac{1}{M_{\zeta}} \nabla L(\xp_1 + \beta \xp_2)$, where $M_{\zeta} := M\zeta^2$, $M > 0$, $\zeta > 0$, and where $d$ and $\beta$ are defined a subsequent section. If the ODE in \cref{eqn:MJODENCVX} is used, we have $u = \hc(\hp(\xp,t)) := -2\bar{d}(t)\xp_2 - \frac{1}{M_{\zeta}}\nabla L(\xp_1 + \bar{\beta}(t)\xp_2)$, where $\bar{d}$ and $\bar{\beta}$ are defined in a subsequent section. If the ODE in \cref{eqn:HBF} is used, then we have $u = \hc(\hp(\xp)) = -\lambda_{\xlogic} \xp_2 - \gamma_{\xlogic} \nabla L(\xp_1)$, with tunable parameters $\lambda > 0$ and $\gamma > 0$.}

%with output given by functions of the state, as defined below and in subsequent sections. The control algorithm $u = \kappa(\hp(\xp,{\color{red}\tau}))$ depends on the ODE involved, and will be defined for specific cases in the subsequent sections. 

For the framework presented in this section, we cope with the trade-off between damping oscillations and converging fast by uniting two control algorithms $\hcq$, where the logic variable $\xlogic \in \xlogicSpace := \{0,1\}$
%{\color{red}, which updates only during jumps,} 
indicates which algorithm is currently being used. The algorithm defined by $\hcone$, which plays the role of the global algorithm in uniting control (see, e.g., \cite{220}), is used far from the minimizer and is designed to quickly get close to the critical point. The algorithm defined by $\hczero$, which plays the role of the local algorithm, is used near the minimizer and is designed to avoid oscillations. The switch between $\hczero$ and $\hcone$ is governed by a {\em supervisory} algorithm implementing switching logic. The supervisor selects between these two optimization algorithms, based on the plant's output and the optimization algorithm currently applied. The design of the logic and parameters of the individual algorithms is done using Lyapunov functions $V_{\xlogic}$, which take different forms depending on the specific optimization methods used for $\hczero$ and $\hcone$. Since the ODE in \cref{eqn:MJODENCVX} is time varying, and since solutions to hybrid systems are parameterized by $(t,j) \in \reals_{\geq 0} \times \naturals$, we employ the state $\tau$ to {\color{red}capture} ordinary time {\color{red}as a state variable, in this way, leading to a time-invariant hybrid system}.

To encapsulate the plant, static state-feedback laws, and the time-varying nature of the ODE in \cref{eqn:MJODENCVX}, we define a hybrid closed-loop system $\HS$ with state $x := \left(\xp, \xlogic, \tau\right) \in \reals^{2n} \times \xlogicSpace \times \reals_{\geq 0}$
%and data $(C,F,D,G)$ 
{\color{red}as follows:
\begin{subequations} \label{eqn:HS-TimeVarying}
	\begin{equation}
		\left.\begin{aligned} 
			\dot{\xp} & = \matt{\xp_2 \\ \hcq(\hp_{\xlogic}(\xp,\tau))}\\
			\dot{\xlogic} & = 0 \\
			\dot{\tau} & = \xlogic
		\end{aligned}\right\} \forall x \in C := C_0 \cup C_1
	\end{equation}
	\begin{equation}
		\left.\begin{aligned}
			\xp^+ & = \matt{\xp_1 \\ \xp_2}\\
			\xlogic^+ & = 1-\xlogic\\
			\tau^+ & = 0
		\end{aligned}\right\} \forall x \in D := D_0 \cup D_1
	\end{equation}
\end{subequations}
Its data is $(C,F,D,G)$ with $F(x) := \left(\xp_2,\kappa_{\xlogic}(\hp_{\xlogic}(\xp,\tau)),0,\xlogic \right)$ and $G(x) := \left(\xp_1,\xp_2,1-\xlogic,0\right)$.}

%\begin{subequations} \label{eqn:HS-TimeVarying}
%	\begin{align}
%		F(x) := & \matt{\matt{\xp_2\\ \kappa_{\xlogic}(\hp_{\xlogic}(\xp,\tau))}\\0\\q} & \forall x \in C := C_0 \cup C_1\\
%		G(x) := & \matt{\xp\\1-\xlogic\\0} & \forall x \in D := D_0 \cup D_1
%	\end{align}
%\end{subequations}
The reason that the state $\tau$ increases at the rate $\xlogic$ during flows and is reset to $0$ during jumps is that when the global algorithm is being used, $\xlogic = 1$ causes ordinary time to increase linearly, starting from $0$, and when the local algorithm is being used, $\xlogic = 0$ causes the time to stay at zero. Such an evolution prevents finite escape time during flows and also ensures that the set of interest is compact. 
	
The sets $C_0$, $C_1$, $D_0$, and $D_1$ are defined as
\begin{subequations} \label{eqn:CAndDGradientsNestNSC}
	\begin{align}
		&C_0 := \U_0 \times \{0\} \times \reals_{\geq 0}, \ C_1 := \overline{\reals^{2n}\setminus \T_{1,0}} \times \{1\} \times \reals_{\geq 0}\\
		&D_0 := \T_{0,1} \times \{0\} \times \reals_{\geq 0}, \ D_1 := \T_{1,0}\times \{1\} \times \reals_{\geq 0},
	\end{align}
\end{subequations}
and where $\U_0$, $\T_{1,0}$, and $\T_{0,1}$ are defined differently, depending on the specific optimization algorithms employed for $\hczero$ and $\hcone$. 
The outputs $\hp_{\xlogic}$ are also defined differently, based on the specific optimization methods used. \Cref{fig:FeedbackDiagram} shows the feedback diagram of this hybrid closed-loop system $\HS$. We denote, for each $\xlogic \in \xlogicSpace = \{0,1\}$, the closed-loop systems resulting from the individual optimization algorithms as $\HS_{\xlogic}$ {\color{red}with state $\left(\xp,\tau\right)$, which are given by
%Namely, the global algorithm $\hcone$ is denoted as $\HS_1$, and the local algorithm $\kappa_0$ is denoted as $\HS_0$. 
\begin{equation} \label{eqn:Hq}
	\left.\begin{aligned}
		\dot{\xp} & = \matt{\xp_2 \\ \hcq(\hp_{\xlogic}(\xp,\tau))}\\
		\dot{\tau} & = 1
	\end{aligned}\right\} \forall \left(\xp,\tau\right) \in \reals^{2n} \times \reals_{\geq 0}.
\end{equation}}

%\begin{figure}[thpb]
%	\centering
%	\setlength{\unitlength}{0.04\textwidth}
%	
%	\begin{picture}(18,12.2)(0,0) % (23,15.2)
%		\normalsize
%%											
%%					\put(0,0){\framebox(18,12.2)}
%%											
%		\put(0,0.5){\includegraphics[scale=0.4,trim={0cm 0cm 0cm 0cm},clip,width=18\unitlength]{Figures/FeedbackDiagram.eps}}
%		\put(6,4.8){{\bf Supervisor}}
%		\put(0.75,3.7){$\dot{\xlogic} = 0 \qquad \qquad \ \dot{\tau} = \xlogic \qquad \ \ (\xp, \xlogic, \tau) \in C := C_0 \cup C_1$}
%		\put(0.75,2.5){$\xlogic^+ = 1- \xlogic \qquad \tau^+ = 0 \qquad (\xp, \xlogic, \tau) \in D := D_0 \cup D_1$}
%		\put(12,8){\bf plant}
%		\put(11.7,10.25){$\dot{\xp}_1 = \xp_2$}
%		\put(11.7,9.25){$\dot{\xp}_2 = u$}
%		\put(2.65,11.05){$\hcone(\hp(\xp,\tau))$}
%		\put(2,9.7){\bf global ($\xlogic = 1$)}
%		\put(2.65,8.5){$\hczero(\hp(\xp,\tau))$}
%		\put(2.2,7.15){\bf local ($\xlogic = 0$)}
%		\put(8.4,8){$\xlogic$}
%		\put(10,10.3){$u$}
%		\put(15.9,10.3){$\hp_{\xlogic}$}
%		\put(0.25,10.3){$\hp_{\xlogic}$}
%	\end{picture}
%	\caption{Feedback diagram of the hybrid closed-loop system $\HS$, in \eqref{eqn:HS-TimeVarying}, uniting global and local optimization algorithms.}
%	\label{fig:FeedbackDiagram}
%\end{figure}

\begin{figure}[thpb]
	\centering
	\setlength{\unitlength}{1.0pc}
	
	\begin{picture}(30.8,12)(0,0) % (23,15.2)
		\normalsize
%													
%							\put(0,0){\framebox(30,13)}
%								
		\put(0,2){\includegraphics[scale=0.2,trim={1.5cm 0cm 0cm 0.8cm},clip,width=11.5\unitlength]{Figures/Surface4.eps}}			
		\put(11.5,0.5){\includegraphics[scale=0.4,trim={0cm 0cm 0cm 0cm},clip,width=19\unitlength]{Figures/FeedbackDiagram2.eps}}
		\put(18.5,4.5){{\bf Supervisor}}
		\put(12.1,3.2){$\ \ \dot{\xlogic} = 0 \qquad \quad \ \dot{\tau} = \xlogic \ \ \ (\xp, \xlogic, \tau) \in C := C_0 \cup C_1$}
		\put(12.1,1.8){$\xlogic^+ = 1- \xlogic \ \ \  \tau^+ = 0 \ \ \ (\xp, \xlogic, \tau) \in D := D_0 \cup D_1$}
		\put(24.4,7.4){\bf plant}
		\put(24.1,9.9){$\dot{\xp}_1 = \xp_2$}
		\put(24.1,8.9){$\dot{\xp}_2 = u$}
		\put(13.9,10.6){$\hcone(\hp_1(\xp,\tau))$}
		\put(13.3,9.1){\bf global ($\xlogic = 1$)}
		\put(13.9,7.5){$\hczero(\hp_0(\xp,\tau))$}
		\put(13.6,5.9){\bf local ($\xlogic = 0$)}
		\put(21,7){$\xlogic$}
		\put(22.1,10.1){$u$}
		\put(28.4,10.1){$\hp_{\xlogic}$}
		\put(11.6,10.1){$\hp_{\xlogic}$}
		\put(7.6,5.3){$\nabla L(\xp_1)$}
		\put(5.5,3.8){$\xp_1^*$}
		\put(6.7,3.3){$\xp_1$}
		\put(8.8,4){$\xp_{1_{\circ}}$}
	\end{picture}
	\caption{Feedback diagram of the hybrid closed-loop system $\HS$ (on the right), in \eqref{eqn:HS-TimeVarying}, uniting global and local optimization algorithms. An example optimization problem to solve is shown on the left and, for this example optimization problem, measurements of the gradient are used for the input of $\hcq$.}
	\label{fig:FeedbackDiagram}
\end{figure}

\subsection{Design}
The sets $\U_0$ and $\T_{1,0}$ need to be designed such that the supervisor can determine when the state component $\xp_1$ is close to the set of minimizers of $L$, which we denote as
\begin{equation} \label{eqn:setOfMinimizers}
	\A_1 := \defset{\xp_1 \in \reals^n}{\nabla L(\xp_1) = 0\!\!},
\end{equation}
without knowledge of $\xp_1^*$ or $L^*$. To facilitate such a design, 
%and to ensure that every maximal solution to $\HS$ is complete, 
we impose the following assumptions\footnote{For the case of strongly convex $L$, nonstrong convexity and quadratic growth is implied, since these are weaker properties than strong convexity \cite{drusvyatskiy2018error} \cite{necoara2019linear} \cite{boyd2004convex}} on $L$.

\begin{assumption} \label{ass:LisNSCVX}
	$L$ is $\mathcal{C}^1$ and (nonstrongly) convex. 
\end{assumption}

\begin{assumption}[Quadratic growth of $L$] \label{ass:QuadraticGrowth}
	{\color{red}The function} $L$ has quadratic growth away from its minima $\A_1$; i.e., there exists $\alpha > 0$ such that\footnote{\Cref{ass:QuadraticGrowth} can be relaxed to a ball $\mathcal{B}^L_{\nu} = \defset{\xp_1 \in \reals^{n}\!\!}{\!\!L(\xp_1) - L^* < \nu\!\!}$ for some $\nu > 0$.}
	\begin{equation} \label{eqn:QuadraticGrowth}
		L(\xp_1) - L^* \geq \alpha \left| \xp_1 \right|_{\A_1}^2 \ \forall \xp_1 \in \reals^{n}.
	\end{equation}
\end{assumption}


\begin{remark}
	\Cref{ass:LisNSCVX}, which is a common assumption used in the analysis of optimization algorithms \cite{boyd2004convex} \cite{nesterov2004introductory}, ensures that the objective function is continuously differentiable, which is necessary for well-posedness of $\HS$. Additionally, the nonstrongly convex property in \cref{ass:LisNSCVX} restricts the objective function to having either a unique minimizer or a continuum of minimizers, rather than multiple isolated minimizers, and is used to construct sets $\U_0$ and $\T_{1,0}$ (defined below).
%	, via upper bounding the Lyapunov functions $V_0$ and $V_1$ -- which take different forms depending on the specific $\hczero$ and $\hcone$ algorithms employed. 
\Cref{ass:QuadraticGrowth} is also used for the construction of $\U_0$ and $\T_{1,0}$, as a means of determining when the state $\xp$ is near the minimizer of $L$, via measurements of the gradient. Such an assumption is also commonly used in the analysis of convex optimization algorithms \cite{drusvyatskiy2018error}, \cite{karimi2016linear}.
\end{remark}

%% Maybe I should do \U_0 first, in a general way, and then \T_{1,0} second....
% Then make sure that I say the constants for \U_0 should ensure that \U_0 is contained in the basin of attraction induced by $\hczero$ -- and it's in a c_0-sublevel set of V_0
% Then make sure I say that \tilde{c}_{1,0} and d_{1,0} should be designed such that, when q = 1, \left| \nabla L(\xp_1) \right| \leq \tilde{c}_{1,0}, and \left|\xp_2\right|^2 \leq d_{1,0}, \xp \in \T_{1,0} is in a c_{1,0} sublevel set of V_1.
The set $\U_0$ is defined, via \cref{def:Convexity}, and\\ \cref{lemma:ConvexSuboptimality}, as follows:
\begin{equation} \label{eqn:U0}
	\U_0 := \defset{\xp \in \reals^{2n}}{\left| \nabla L(\xp_1) \right| \leq \tilde{c}_0,\frac{1}{2} \left|\xp_2\right|^2 \leq d_0}
\end{equation}
where the parameters $\tilde{c}_0 > 0$ and $d_0 > 0$ are designed so that $\U_0$ is in the region where $\hczero$ is used. 

The set $\T_{1,0}$ is defined, via \cref{def:Convexity}, and \cref{lemma:ConvexSuboptimality}, as follows:
\begin{equation} \label{eqn:T10}
	\T_{1,0} := \defset{\xp \in \reals^{2n}}{\left| \nabla L(\xp_1) \right| \leq \tilde{c}_{1,0}, \left|\xp_2\right|^2 \leq d_{1,0}} 
\end{equation}
where the parameters $\tilde{c}_{1,0} \in (0, \tilde{c}_0)$ and $d_{1,0} \in (0, d_0)$ are designed such that $\T_{1,0}$ is contained in the interior of $\U_0$. When $\xlogic = 1$, $\left| \nabla L(\xp_1) \right| \leq \tilde{c}_{1,0}$, and $\left|\xp_2\right|^2 \leq d_{1,0}$, the supervisor will switch from the global algorithm $\hcone$ to the local algorithm $\hczero$.  The constants $\tilde{c}_0$, $\tilde{c}_{1,0}$, $d_0$, and $d_{1,0}$ comprise the hysteresis necessary to avoid chattering at the switching boundary. Examples illustrating the design of $\U_0$ and $\T_{1,0}$ for specific cases of $\hczero$ and $\hcone$ are presented in \Cref{sec:SpecificCases}.

%% Then, here I should say that since \U_0 is contained in the basin of attraction induced by $\hczero$, then T_{0,1} should be designed such that it is a closed complement of the c_0-sublevel set of V_0. 
% Also, it should be designed such that the algorithm doesn't need to know L^* and z_1^* -- suggest any such terms in V can be lower bounded using the assumptions above, for example.
The set $\T_{0,1}$ should be designed such that the supervisor can determine that the state $\xp$ is far from the minimizer, when $\xp \in \T_{0,1}$ and $\xlogic = 0$, and make the switch back to $\hcone$ to ensure that the state $\xp$ reaches the neighborhood of the minimizer in finite time. Additionally, the set $\T_{0,1}$ should be designed such that, when used in combination with $\U_0$ and $\T_{1,0}$ to define \cref{eqn:CAndDGradientsNestNSC}, each solution $x$ to the hybrid closed-loop algorithm $\HS$ jumps no more than twice, and the set of interest is guaranteed to be at least weakly forward invariant.

%To ensure that the set $\T_{0,1}$ satisfies the above properties, it should be defined as the (closed) complement of the $c_0$-sublevel set of $V_0$ with level $\hat{c}_0 > c_0$. As $V_0$ can potentially have terms containing $L(\xp_1) - L^*$ or $\xp_1^*$, then when constructing $\T_{0,1}$ such terms can be lower bounded by utilizing \cref{ass:QuadraticGrowth} and/or including additional mild assumptions on $L$ or $\nabla L$, as shown in the special cases in \Cref{sec:SpecificCases}.

% Include the assumptions that lead to the general results (i.e., suboptimality)
To ensure that the hybrid closed-loop system $\HS$ in \cref{eqn:HS-TimeVarying}, with $C$ and $D$ defined via \cref{eqn:CAndDGradientsNestNSC}, is well-posed, and to ensure that every maximal solution to the hybrid closed-loop system $\HS$ is complete, we impose the following assumptions on the set $\T_{0,1}$ and the static state-feedback laws $\kappa_{\xlogic}(\hp_{\xlogic}(\xp,\tau))$.

\begin{assumption}[Closed sets and continuous static state-feedback laws]\label{ass:AssumpsForHBC}
	\begin{enumerate}[label={(C\arabic*)},leftmargin=*]
		\item \label{item:C1} The set $\T_{0,1}$ is closed;
		\item \label{item:C2} {\color{red}The map $\xp \mapsto F_P(\xp,\kappa_{\xlogic}(\hp_{\xlogic}(\xp,\tau)))$, in \cref{eqn:HBFplant-dynamicsTR} with $u = \kappa(\hp(\xp,\tau))$, is Lipschitz continuous with constant $M_{{\color{red}\kappa}} > 0$, namely,
		\begin{equation}
			\left|F_P(\xp,\hcq(\hp_{\xlogic}(\xp,\tau_1))) - F_P(v,\hcq(\hp_{\xlogic}(v,\tau_2))) \right| \leq M_{\kappa} \left|\xp - v\right|
		\end{equation}
		for all $\xp,v \in \reals^{2n}$ and all $\tau_1,\tau_2 \in \reals_{\geq 0}$.}
%		
%		{\color{red}Letting $\chi := \left(\xp,\tau\right)$,} The feedback laws $\xp \mapsto \hcq(\hp_{\xlogic}(\xp,\tau))$ in \cref{eqn:HS-TimeVarying} are Lipschitz continuous with constant $M_{{\color{red}\kappa}} > 0$, namely,
%		\begin{equation}
%			\left|\kappa_{\xlogic}(\hp_{\xlogic}(\chi_1)) - \kappa_{\xlogic}(\hp_{\xlogic}(\chi_2))\right| \leq M_{{\color{red}\kappa}} {\color{red}\left|\chi_1 - \chi_2\right|}
%		\end{equation}
%	for all {\color{red}$\chi_1, \chi_2 \in \reals^{2n} \times \reals_{\geq 0}$}. 
	\end{enumerate}
\end{assumption}

\begin{remark} 
	Whereas $C$ is closed by construction, \cref{item:C1} is needed to ensure that the set $D$ is closed. \Cref{item:C2} is used to ensure that the map $x \mapsto F(x)$ is continuous. The closure of $C$ and $D$ and the continuity of $F$ and $G$ are required for $\HS$ to be well-posed which, in turn, leads to robustness of the asymptotic stability our framework guarantees, as stated in results to follow. Additionally, \cref{item:C2} is an assumption commonly used in nonlinear analysis to ensure that the differential equations of the individual optimization algoriths, for example those in \cref{eqn:MJODE,eqn:MJODENCVX,eqn:HBF}, do not have solutions that escape in finite time, which is used to guarantee the existence of solutions to $\HS_{\xlogic}$ \cite[Theorem~3.2]{khalil2002nonlinear}. 
\end{remark}

\subsection{Basic Properties of $\HS$} \label{sec:BasicProperties}
Under \cref{ass:LisNSCVX,ass:AssumpsForHBC}, the hybrid closed-loop system $\HS$ in \cref{eqn:HS-TimeVarying}, with $C$ and $D$ defined via \cref{eqn:CAndDGradientsNestNSC}, is well-posed as it satisfies the hybrid basic conditions, as demonstrated in the following lemma. 
\begin{lemma}[Well-posedness of $\HS$] 
	\label{lemma:HBCC}
	Let $L$ satisfy \cref{ass:LisNSCVX,ass:AssumpsForHBC}. Then the hybrid closed-loop system $\HS$ satisfies the hybrid basic conditions, as listed in \cref{def:HBCs}.
\end{lemma}

\begin{proof}
	The sets $\U_0$ and $\T_{1,0}$ are closed by construction, and by \cref{item:C1} $\T_{0,1}$ is closed. Therefore, the sets $D_0$, $D_1$, $C_0$, and $C_1$ are closed. Since $D$ is a finite union of finite sets, then $D$ is closed, and since $C$ is a finite union of finite and closed sets, then $C$ is also closed. 
	
	By construction the map $x \mapsto \f(x)$ is continuous since, by \cref{item:C2}, 
%	$\xp \mapsto \hcq(\hp_{\xlogic}(\xp, \tau))$ 
	{\color{red}$\xp \mapsto F_P(\xp,\kappa_{\xlogic}(\hp_{\xlogic}(\xp,\tau)))$}
	is Lipschitz continuous. The map $\g$ satisfies \cref{item:A3} by construction. 
\end{proof}

As mentioned above, a hybrid closed-loop system $\HS$ that satisfies the hybrid basic conditions is well-posed. Such a property is important because when the hybrid closed-loop system $\HS$ is well-posed and has a compact pre-asymptotically stable set, we can show that such pre-asymptotic stability is robust to small perturbations \cite[Theorem~7.21]{65}. In the case of gradient-based algorithms, for instance, such perturbations can take the form of small noise in measurements of the gradient.

When \cref{ass:LisNSCVX,ass:QuadraticGrowth,ass:AssumpsForHBC} hold, then every maximal solution to the hybrid closed-loop system $\HS$ is complete and bounded. 

\begin{proposition}[Existence of solutions to $\HS$]
	\label{prop:ExistenceC}
	Let $L$ satisfy \cref{ass:LisNSCVX,ass:QuadraticGrowth} and let the set $\T_{0,1}$ and the
%	static state-feedback laws ${\color{red}\xp \mapsto } \hcq(\hp_{\xlogic}(\xp,{\color{red}\tau}))$
	{map \color{red}$\xp \mapsto F_P(\xp,\kappa_{\xlogic}(\hp_{\xlogic}(\xp,\tau)))$} {\color{red}, $\xlogic \in \{0,1\}$,} satisfy \cref{ass:AssumpsForHBC}. Furthermore, let $\U_0$ and $\T_{1,0}$ be defined via \cref{eqn:U0} and \cref{eqn:T10}, respectively. Then, each {\color{red}maximal solution\\ $(t,j) \mapsto x(t,j) = (\xp_1(t,j),\xp_2(t,j),\xlogic(t,j),\tau(t,j))$ to $\HS$ is bounded and complete.} 
\end{proposition}

\begin{proof}
	Since \cref{ass:LisNSCVX,ass:AssumpsForHBC} hold, then $\HS$ is well-posed. For points $x \in C \setminus D$, the tangent cone $T_C(x) \in \reals^{2n}$. Therefore $F$ satisfies (VC) of \cref{prop:SolnExistence}, and nontrivial solutions exist for every initial point in $C \cup D$.
	To prove that item (c) of \cref{prop:SolnExistence} does not hold, we need to show that $G(D) \subset C \cup D$. For $D$, as defined in \cref{eqn:CAndDGradientsNestNSC}, $G(D)$ is as follows
	\begin{equation} \label{eqn:CG(D)}
		G(D)  = \left(\T_{0,1} \times \{1\} \times \reals_{\geq 0} \right) \cup \left(\T_{1,0} \times \{0\} \times \reals_{\geq 0} \right) 
	\end{equation}	
	Notice that $\left(\T_{1,0} \times \{0\} \times \reals_{\geq 0} \right) \subset C_0$ and $\left(\T_{0,1} \times \{1\} \times \reals_{\geq 0} \right) \subset C_1$. Therefore,\\ $G(D) \subset C$, and this means also that $G(D) \subset C \cup D$. Therefore, item (c) of \cref{prop:SolnExistence} does not hold. Then it remains to prove that item (b) does not apply. 
	
	Since by \cref{item:C2}, 
%	$\xp \mapsto \hcq(\hp_{\xlogic}(\xp,\tau))$ 
	{\color{red}$\xp \mapsto F_P(\xp,\kappa_{\xlogic}(\hp_{\xlogic}(\xp,\tau)))$} is Lipschitz continuous, {\color{red}and since $\tau$ increases linearly},
%	{\color{red}and since $\dot{\tau} = 1$,} 
	then by \cite[Theorem~3.2]{khalil2002nonlinear}, 
%	${\color{red}\dot{\chi}} = F_P(\xp,\hcq(\hp_{\xlogic}(\xp,\tau)))$ 
	{\color{red}there is} no finite time escape for $\HS_{\xlogic}${\color{red}, defined via \cref{eqn:Hq}}. Therefore, every maximal solution {\color{red}$(\xp,\tau)$} to the individual optimization algorithms $\HS_{\xlogic}$ is complete, with unique solutions. Therefore, this means $\dot{x} = F(x)$ has no finite time escape from $C$ for $\HS$, as $\xlogic$ does not change in $C$ and as $\tau$ is bounded in $C$, namely, $\tau$ -- which is always reset to $0$ in $D$ -- increases linearly in $C_1$ and remains at $0$ in $C_0$. Moreover, the jump map $G$, defined via \cref{eqn:HS-TimeVarying}, shows that when the system is in $D$, $\xp$ does not change, $\xlogic$ is reset from $0$ to $1$ or vice versa, and $\tau$ is always reset to $0$. Therefore, by the construction of $\g$, and by the properties of solutions to
%	${\color{red}\dot{\chi}} = F_P(\xp,\hcq(\hp_{\xlogic}(\xp, \tau)))$
	{\color{red}$\HS_{\xlogic}$},
%	{\color{red}$\dot{\xp} = F_P(\xp,\kappa_{\xlogic}(\hp_{\xlogic}(\xp,\tau)))$},
	there is no finite time escape from $C \cup D$, for solutions to $\HS$. Therefore, item (b) from  \cref{prop:SolnExistence} does not hold. This means only item (a) is true, and every maximal solution $x$ to $\HS$ is {\color{red}bounded and} complete. 
\end{proof}

As evidenced by \cref{def:Convexity} in \Cref{sec:Preliminaries}, the set of nonstrongly convex functions includes a subset of functions $L$ which have a connected continuum of minimizers, with the most extreme case being linear functions \cite{boyd2004convex} \cite{nocedal2006numerical}. Therefore, we make the following assumption\footnote{When $L$ is strongly convex, then $L$ has a single minimizer, which implies compact and connected $\A_1$.}, used in the results to follow.  
\begin{assumption}[Compact and connected $\A_1$] 
	\label{ass:CompactAndConnected}	
	The set $\A_1$, defined in \cref{eqn:setOfMinimizers}{\color{red},} is compact and connected.
	%	\begin{enumerate}[label={(C\arabic*)},leftmargin=*]
	%		\item \label{item:C1} $\A_1$, defined in \eqref{eqn:setOfMinimizers}, is compact and connected;
	%		\item \label{item:C2} $L$ is positive definite with respect to $\A_1$.
	%	\end{enumerate}
\end{assumption}

%To establish UGAS of the set of interest for the hybrid closed-loop algorithm $\HS$, we impose the following assumptions on the closed-loop algorithms $\HS_0$ and $\HS_1$.
%\begin{assumption}[Assumptions on asymptotic stability and attractivity] \label{ass:UGAS}
%	\begin{enumerate}[label={(U\arabic*)},leftmargin=*]
%		
%		
%	\end{enumerate}
%\end{assumption}

To establish uniform global asymptotic stability of the set of interest for the hybrid closed-loop algorithm $\HS$, we impose the following assumptions on the closed-loop algorithms $\HS_{\xlogic}$ in \cref{eqn:Hq}.
We also make assumptions about the sets $\U_0$, $\T_{1,0}$, and $\T_{0,1}$, to ensure that each solution $x$ to the hybrid closed-loop algorithm $\HS$ jumps no more than twice, and ensure that the set of interest is guaranteed to be at least weakly forward invariant for $\HS$.

\begin{assumption}[{\color{red}Assumptions on asymptotic stability and attractivity}] \label{ass:UnitingControl}\\
	Given $\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}} \in \reals^{2n} {\color{red}\times \reals_{\geq 0}}$ and a plant defined via \cref{eqn:HBFplant-dynamicsTR} with $\yp = \hp{\color{red}_{\xlogic}}(\xp)$, {\color{red}given $\tilde{c}_0 > 0$ and $d_0 > 0$ defining the closed set $\U_0 \in \reals^{2n}$ via} \cref{eqn:U0}, the interior of which contains an open neighborhood of $\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}} \in \reals^{2n} {\color{red}\times \reals_{\geq 0}}$, and {\color{red}given $\tilde{c}_{1,0} \in (0,\tilde{c}_0)$ and $d_{1,0} \in (0,d_0)$ defining the closed set $\T_{1,0} \subset \U_0$ via} \cref{eqn:T10}, the following conditions {\color{red}hold:} 
	\begin{enumerate}[label={(UC\arabic*)},leftmargin=*]
		\item \label{item:UC1} The closed-loop algorithm $\HS_1$, resulting from $\hcone$, has the set $\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}}$ uniformly globally attractive, namely, every maximal solution {\color{red}$\chi := (\xp,\tau)$} to $\HS_1${\color{red}, given by \cref{eqn:Hq} with $u = \hcone(\hp_1(\xp,\tau))$,} is complete and for each $\eps > 0$ and $r > 0$ there exists $T > 0$ such that, for any solution {\color{red}$\chi$} to $\HS_1$ with $\left|{\color{red}\chi}(0)\right|_{\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}}} \leq r$, $t \in \dom {\color{red}\chi}$ and $t \geq T$ imply\footnote{{\color{red} Although we employ $\tau$ as a state to capture ordinary time, we can use just $t$ to parameterize solutions.}} $\left|{\color{red}\chi}(t)\right|_{\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}}} \leq \eps$;
		\item \label{item:UC2} There exist positive constants $\tilde{c}_1 \in (0,\tilde{c}_{1,0})$ and $d_1 \in (0,d_{1,0})$ such that the closed set $\T_{1,0}$ satisfies
		%		Constants $\delta_0 > 0$, $\delta_0^{\tilde{c}}$, and $\delta_0^d$, and a 
		%		A closed set $\T_{1,0}$ satisfying
		%		\begin{equation}
		%			\left(\A_1 + \left(\tilde{c}_1 + \delta_0^{\tilde{c}}\right) \ball \right) \times \left(\{0\} + \left(d_1 + \delta_0^d\right) \ball\right) \subset \T_{1,0}, \qquad \T_{1,0} + 2\delta_0 \ball \subset \U_0
		%		\end{equation}
		\begin{equation} \label{eqn:c1d1Set}
%			\left(\A_1 + \left(\tilde{c}_1 + \delta_0^{\tilde{c}}\right) \ball \right) \times \left(\{0\} + \left(d_1 + \delta_0^d\right) \ball\right) \subset \T_{1,0}
			\left(\A_1 + \tilde{c}_1 \ball \right) \times \left(\{0\} + d_1 \ball\right) \subset \T_{1,0}
		\end{equation}
		and each solution to {\color{red}$\HS_0$} in \cref{eqn:Hq} with initial condition in $\T_{1,0} {\color{red}\times \reals_{\geq 0}}$, resulting from applying $\hczero$, remains in $\U_0$;
		\item \label{item:UC3} The closed-loop algorithm $\HS_0$, resulting from $\hczero$, has a set $\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}}$ uniformly globally asymptotically stable, namely, every maximal solution {\color{red}$\chi$} to $\HS_0${\color{red}, given by \cref{eqn:HBFplant-dynamicsTR} with $u = \hczero(\hp_0(\xp,\tau))$,} is complete, $\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}}$ is uniformly globally attractive for $\HS_0$, and there exists a class-$\mathcal{K}_{\infty}$ function $\alpha$ such that any solution {\color{red}$\chi$} to $\HS_0$ satisfies $\left|{\color{red}\chi}(t)\right|_{\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}}} \leq \alpha \left(\left|{\color{red}\chi}(0)\right|_{\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}}}\right)$ for all $t \in \dom {\color{red}\chi}$.
		\item \label{item:UC4} There exists a constant $\delta_0 > 0$ and a closed set $\T_{0,1} + 2\delta_0 \ball \subset \overline{\reals^{2n}\setminus \U_0}$ such that when $\xp \in \T_{0,1}$ and $\hczero$ is currently being used, {\color{red}the hybrid closed-loop algorithm $\HS$ assigns $u$ to $\hcone$}.
	\end{enumerate}
\end{assumption}

\begin{remark}
	\Cref{ass:CompactAndConnected} ensures that the set $\A$ (defined below) is compact, which is required in the forthcoming analysis of the stability properties of $\HS$. \Cref{item:UC1,item:UC3} of \cref{ass:UnitingControl} ensure that $\HS_1$ and $\HS_0$ have the desired attractivity and stability properties, respectively, to establish the stability of the hybrid closed-loop algorithm $\HS$. Such assumptions are reasonable in light of the numerous results in the literature for gradient-based optimization algorithms, cited in \Cref{sec:Intro}. Furthermore, the conditions in \Cref{ass:UnitingControl} are similar to conditions imposed in \cite{220} for general uniting control algorithms. 
	\Cref{item:UC1} ensures that solutions {\color{red}$\left(\xp,\tau\right)$ starting with $\xp$ in $\U_0$, with $\xlogic = 0$ and $\tau \in \reals_{\geq 0}$, stay in $\U_0$ and converge to $\A_1 \times \{0\} \times \reals_{\geq 0}$} under the affect of $\hczero$.
	\Cref{item:UC4} guarantees that solutions starting with the state $\xp \in T_{0,1}$ and with $\xlogic = 0$ triggers a jump resetting $\xlogic$ to $1$. \Cref{item:UC3} guarantees that, after such a jump, $\xp$ reaches $\T_{1,0}$ in finite time with $\hcone$ applied. 
	\Cref{item:UC2} ensures that solutions from $\T_{1,0}$ under the effect of $\hczero$ cannot reach the boundary of $\U_0$.
\end{remark}

% Put general result here
The following theorem establishes that the hybrid closed-loop system $\HS$ in \cref{eqn:HS-TimeVarying}-\cref{eqn:CAndDGradientsNestNSC} has the set
\begin{equation} \label{eqn:SetOfMinimizersHS-NSCVX}
	\A := \defset{\xp \in \reals^{2n}}{\nabla L(\xp_1) = \xp_2 = 0} \times \{0\} \times \{0\} = \A_1 \times \{0\} \times \{0\} \times \{0\}
\end{equation}
uniformly globally asymptotically stable. The penultimate component $\{0\}$ in $\A$ is due to the logic state ending with the value $\xlogic = 0$, namely using $\kappa_0$ as the state $\xp$ reaches the set of minimizers of $L$. The last component $\{0\}$ in $\A$ is due to $\tau$ being set to and then staying at zero when the supervisor switches to $\hczero$.  To prove this result, we use an invariance principle. 

\begin{theorem}[Uniform global asymptotic stability of $\A$ for $\HS$] \label{thm:GASGen}
	Let $L$ satisfy \cref{ass:LisNSCVX,ass:QuadraticGrowth,ass:CompactAndConnected}, let the
%	feedback laws $\xp \mapsto \hcq(\hp_{\xlogic}(\xp,\tau))$ {\color{red}in \cref{eqn:HS-TimeVarying}} 
	{\color{red}map $\xp\mapsto F_P(\xp,\kappa_{\xlogic}(\hp_{\xlogic}(\xp,\tau)))$, $\xlogic \in \{0,1\}$, in \cref{eqn:HBFplant-dynamicsTR}}
	satisfy \cref{ass:AssumpsForHBC}, let the closed-loop optimization algorithms $\HS_{\xlogic}$ {\color{red}in \cref{eqn:Hq}} and the sets $\U_0$, $\T_{1,0}$, and $\T_{0,1}$ satisfy \cref{ass:UnitingControl}. Additionally, let $\delta_0 > 0$, $\tilde{c}_{1,0} \in (0,\tilde{c}_0)$, $\tilde{c}_1 \in (0,\tilde{c}_{1,0})$, $d_{1,0} \in (0,d_0)$, and $d_1 \in (0,d_{1,0})$. Then, the set $\A$, defined via \eqref{eqn:SetOfMinimizersHS-NSCVX}, is uniformly globally asymptotically stable for $\HS$ {\color{red}given in \cref{eqn:HS-TimeVarying}-\cref{eqn:CAndDGradientsNestNSC}}.
\end{theorem}

\begin{proof}
	The hybrid closed-loop algorithm $\HS$ satisfies the hybrid basic conditions by \cref{lemma:HBCC}, satisfying the first assumption of \cref{thm:hybrid Lyapunov theorem}. Furthermore, every maximal solution $(t,j) \mapsto x(t,j) = (\xp_1(t,j), \xp_2(t,j), \xlogic(t,j),\tau(t,j))$ to $\HS$ for \cref{eqn:HS-TimeVarying}-\cref{eqn:CAndDGradientsNestNSC} is complete and bounded by \cref{prop:ExistenceC}. By \cref{ass:CompactAndConnected}, $\A_1$ is compact and connected.
	Therefore, $\A$, defined via \cref{eqn:SetOfMinimizersHS-NSCVX}, is compact by construction, and $\U = \reals^{2n}$ contains a nonzero open neighborhood of {\color{red}$\A_1$}.
	
	To prove the attractivity of $\A$, we use a trajectory based approach which uses the properties of the individual optimization algorithms $\HS_0$ and $\HS_1$. The possible trajectory types for $\HS$ are:
	
	\begin{enumerate}[label={\arabic*)},leftmargin=*]
		\item Trajectories that start in $C_0$, namely, such that $\xp(0,0) \in \U_0$, $\xlogic(0,0) = 0$, and $\tau(0,0) = 0$;
		\item Trajectories that start in the interior of $D_1$, namely, such that $\xlogic(0,0) = 1$, $\tau(0,0) = 0$, and either $\left|\nabla L(\xp_1(0,0))\right| < \tilde{c}_{1,0}$, $\left|\xp_2(0,0)\right|^2 \leq d_{1,0}$ or $\left|\nabla L(\xp_1(0,0))\right| \leq \tilde{c}_{1,0}$, $\left|\xp_2(0,0)\right|^2 < d_{1,0}$;
%		\item Trajectories that start on the boundary between $C_1$ and $D_1$, namely, such that $\left|\nabla L(\xp_1(0,0))\right| = \tilde{c}_{1,0}$, $\left|\xp_2(0,0)\right|^2 = d_{1,0}$, $\xlogic(0,0) = 1$, and $\tau(0,0) = 0$; 
		\item Trajectories that start in the interior of $C_1$, namely, such that $\xlogic(0,0) = 1$, $\tau(0,0) = 0$, and either $\left|\nabla L(\xp_1(0,0))\right| > \tilde{c}_{1,0}$, $\left|\xp_2(0,0)\right|^2 \geq d_{1,0}$ or $\left|\nabla L(\xp_1(0,0))\right| \geq \tilde{c}_{1,0}$, $\left|\xp_2(0,0)\right|^2 > d_{1,0}$;
		\item Trajectories that start in $D_0$, namely, such that $\xp(0,0) \in \T_{0,1}$, $\xlogic(0,0) = 0$, $\tau(0,0) = 0$.
	\end{enumerate}
%	Due to the construction of $\g$, the value of $\xp$ does not change during jumps. Furthermore, by the construction of $D$ in \cref{eqn:CAndDGradientsNestNSC}, with $\tilde{c}_0 > \tilde{c}_{1,0}$ and $d_0 > d_{1,0}$, 
%	
%	
%	solutions that enter $D_0$ only jump once, and never enter $D_0$ again. This is also the case for $D_1$. Due to these same properties, solutions never jump directly from $D_0$ to $D_1$ or vice versa, but enter $C$ and flow before jumping again. Therefore, solutions to $\HS$ never have more than two jumps.
	
	First we analyze trajectories of type 1). By \cref{item:UC4}, the set $\T_{0,1} + 2\delta_0 \ball \subset \overline{\reals^{2n}\setminus\U_0}$. Therefore, $\U_0$ does not share a boundary with $\T_{0,1}$ and, when $\xp(0,0) \in \U_0$, including on the boundary of $\U_0$, then by \cref{item:UC1} of \cref{ass:UnitingControl} solutions only flow using $\hczero$ for all future hybrid time in its domain. 
		
%	By \cref{item:S1}, when $\xp(0,0) \in \U_0$, it is in a $c_0$-sublevel set of $V_0$. Furthermore, since $\hat{c}_0 > c_0$ and $\T_{0,1}$ is a closed complement of the $c_0$-sublevel set of $V_0$ with level $\hat{c}_0$, such that any $L^*$ and $\xp^*$ terms are lower bounded via $\nabla L$ or a constant, by \cref{item:S3}. Consequently, $C_0$ does not share a boundary with $D_0$. Therefore, since by \cref{item:U2} The set $\A_1 \times \{0\}$ uniformly globally asymptotically stable for the closed-loop algorithm $\HS_0$, then all solutions starting in $C_0$ never jump, but instead only flow using $\hczero$. Therefore, the set $\A$ is attractive, for all trajectories of type 1).
	
	Next we analyze trajectories of type 2). Due to the construction of $G$, defined via \cref{eqn:HS-TimeVarying}, when $\xp(0,0) \in D_1$ and $\xlogic = 1$, then the algorithm jumps, resetting $\xlogic$ to $0$ and assigning $u$ to $\hczero$ while $\xp$ does not change. After such a jump, due to the construction of $D_1$, defined via \cref{eqn:CAndDGradientsNestNSC} with $0 < \tilde{c}_{1,0} < \tilde{c}_0$ and $0 < d_{1,0} < d_0$, and due to \cref{item:UC1,item:UC2} of \cref{ass:UnitingControl}, the state $\xp$ remains in $\U_0$ due to the affect of $\hczero$ and from such a point the solution exhibits the same behavior as for trajectories of type 1). 
		
%	When the state $\xp$ starts in the interior of $D_1$ while $\hcone$ is currently being used, then $\xp$ is near the minimizer and the algorithm jumps, resetting $\xlogic$ to $0$ and assigning $u$ to $\hczero$ while $\xp$ does not change. Then, the state $\xp$ is in the interior of $C_0$ since, by \cref{item:S2} $\T_{1,0}$, is contained in the interior of $\U_0$, and from such a point the solution follows the behavior of type 1) trajectories. Therefore, the set $\A$ is attractive, for all trajectories of type 2).
	
%	Next we analyze trajectories of type 3). Such a trajectory starts with $\xp(0,0)$ on the boundary between $C_1$ and $D_1$. On such a boundary, when $\xlogic = 1$, the following two cases are possible. The algorithm could jump first, or the algorithm could flow first, using $\hcone$, and then jump. In the first case, the solution exhibits the same behavior as for trajectories of type 2). In the latter case, the state $\xp$ reaches $D_1$ in finite time since, by \cref{item:UC3} and \cref{item:U1}, $\A_1 \times \{0\}$ is uniformly globally attractive for $\HS_1$, then the state $\xp$ reaches $\left(\A_1 + \tilde{c}_1 \ball \right) \times \left(\{0\} + d_1 \ball\right)$ after finite flow time or as $t$ tends to $\infty$, from points not in $\left(\A_1 + \tilde{c}_1 \ball \right) \times \left(\{0\} + d_1 \ball\right)$. After such a time, the algorithm jumps, with the solution exhibiting the same behavior as for trajectories of type 2).
	
	Then, we analyze trajectories of type 3). When $\xp(0,0)$ starts in $C_1$, then the algorithm flows using $\hcone$. Then, the state $\xp$ reaches $D_1$ in finite time since, by \cref{item:UC3}, $\A_1 \times \{0\} {\color{red}\times \reals_{\geq 0}}$ is uniformly globally attractive for $\HS_1$ and therefore the state $\xp$ reaches $\left(\A_1 + \tilde{c}_1 \ball \right) \times \left(\{0\} + d_1 \ball\right)$ after finite flow time or as $t$ tends to $\infty$, from points starting in $\overline{\reals^{2n}\setminus \left(\left(\A_1 + \tilde{c}_1 \ball \right) \times \left(\{0\} + d_1\ball\right)\right)}$. After such a finite flow time, the algorithm jumps, with the solution exhibiting the same behavior as for trajectories of type 2). 
	
	Finally, we analyze trajectories of type 4). By \cref{item:UC4}, when $\xp(0,0)$ is in $\T_{0,1}$, and $\xlogic = 0$, then the algorithm jumps, resetting $\xlogic$ to $1$ and updating $u$ to $\hcone$. Then, the state $x$ is in $C_1$ and from such a point the solution  exhibits exhibits the same behavior as for trajectories of type 3). 
	
%	Since by \cref{item:S3}, $\T_{0,1}$ is the closed complement of the $c_0$-sublevel set of $V_0$ with level $\hat{c}_0 > c_0$, such that any $L^*$ and $\xp^*$ terms are lower bounded via $\nabla L$ or a constant, then $D_0$ does not share a boundary with $C_0$. Consequently, when the state $\xp(0,0)$ is in $D_0$, the hybrid closed-loop algorithm can only jump first, resetting $\xlogic$ to $1$ and assigning $u$ to $\hcone$ while $\xp$ remains the same. From such a point, the solution follows the behavior of type 4) trajectories. Therefore, the set $\A$ is attractive, for all trajectories of type 5). 
	
	Due to the behaviors of trajectories 1)-5) as described above, and due to the properties in \cref{ass:UnitingControl}, every maximal solution $x$ to $\HS$ exhibits no more than two jumps. Since, additionally, every trajectory of the hybrid closed-loop algorithm $\HS$ ends with $\xlogic = 0$, and since $\tau$ is set to and then stays at zero when the supervisor switches to $\hczero$, then every bounded and complete solution to $\HS$ converges to $\A$. Generally, the Lyapunov theorem and the invariance principle prove global pre-asymptotic stability. But since by \cref{prop:ExistenceC} every maximal solution is complete, then $\A$, defined via \cref{eqn:SetOfMinimizersHS-NSCVX} is uniformly globally asymptotically stable for $\HS$.  
\end{proof}

The framework defined in \cref{eqn:HS-TimeVarying}-\cref{eqn:CAndDGradientsNestNSC} allows for combinations of different methods, including Nesterov's algorithm, the heavy ball method, classic gradient descent, and the triple momentum method \cite{van2017fastest} \cite{sun2020high}, to name a few examples. In the next section, we present specific cases utilizing combinations of Nesterov's algorithm and the heavy ball algorithm. 
